The vanishing relaxation time behavior of multi-term nonlocal Jordan-Moore-Gibson-Thompson equations

The family of Jordan-Moore-Gibson-Thompson (JMGT) equations arises in nonlinear acoustics when a relaxed version of the heat flux law is employed within the system of governing equations of sound motion. Motivated by the propagation of sound waves in complex media with anomalous diffusion, we consider here a generalized class of such equations involving two (weakly) singular memory kernels in the principal and non-leading terms. To relate them to the second-order wave equations, we investigate their vanishing relaxation time behavior. The key component of this singular limit analysis are the uniform bounds for the solutions of these nonlinear equations of fractional type with respect to the relaxation time. Their availability turns out to depend not only on the regularity and coercivity properties of the two kernels, but also on their behavior relative to each other and the type of nonlinearity present in the equations.

==> testing_psi_tt_Deltapsi_GFE.tex <==
\newpage
\vspace*{2mm}
{
\centering
\textbf{THE CASE $\boldsymbol{\ttb \frakKtwo=\delta_0}$} \\[4mm]
}
In this case, the equations can be written as
\begin{equation}
	\taua \frakKone *(\utt-c^2\Delta u)_t+ \aaa \utt-c^2\bbb\Delta u - \delta \Delta \ut +\calN= f
\end{equation}
and the vanishing limit in $\tau$ leads to classical damped integer-order models of nonlinear acoustics. We investigate separately Westervelt-type (in pressure form) and Blackstock--Kuznetsov-type nonlinearities below, as they will require different assumptions on the data.
\section{Analysis with Westervelt-type nonlinearities} \label{Sec:WestType}
We study the linearized equation
\begin{equation} \label{GFE_type_eq}
\taua \frakKone *(\utt-c^2\Delta u)_t+ (\aaa(x,t) \ut)_t-c^2\Delta u - \delta \Delta \ut = f
\end{equation}
where in this section the coefficient $\aaa$ serves as a placeholder for $1+2k_1 u$. The main idea in the analysis is to test this equation with
 \[y= \utt-c^2\Delta u.\]
An advantage of this combined testing procedure is that we only need the following coercivity assumption on $\frakKone$: 
 \begin{equation}\label{eqn:Alikhanov_1}
 	\int_0^{t'} \int_0^t\frakKone(t-s) y'(s)\ds \,y(t)\dt \geq - C_{\frakKone} |y(0)|^2, \quad y\in X_{\frakKone}^2, 
 \end{equation}
where we recall that the space $X_{\frakKone}^2$ is defined in \eqref{def_Xfp}. We outline here the main arguments and then justify them rigorously below.\\
\indent In terms of assumptions on the variable coefficient, it should be smooth, bounded uniformly in $\tau$, and non-degenerate. That is, we assume that 
\begin{equation}
	\aaa \in L^\infty(0,T; L^\infty(\Omega)) \cap W^{1,\infty}(0,T; L^4(\Omega))
\end{equation}
and that there exist $\ulaaa$, $\olaaa>0$, independent of $\tau$, such that
\begin{equation} \label{nondeg_aaa}
	\ulaaa < \aaa(x,t) < \olaaa \quad \text{for all} \ (x,t) \in \Omega \times (0,T).
\end{equation} 
Let $f \in L^2(0,T; L^2(\Omega))$. Testing the (semi-discrete) problem with $y(t)=\utt-c^2\Delta u$ and using the above assumption on the kernel gives
\begin{equation}
	\begin{aligned}
	&\inttO	(\aaa \utt-c^2\Delta u - \delta \Delta \ut)(\utt-c^2\Delta u)\dxs\\
	 \leq& \,- \inttO \aaa_t \ut (\utt-c^2\Delta u)\dxs+\inttO f (\utt-c^2\Delta u)\dxs + \taua C_{\frakKone} \|\utt(0)-c^2 \Delta u(0)\|^2_{L^2}.
	\end{aligned}
\end{equation}
From here we have
\begin{equation}
	\begin{aligned}
&\begin{multlined}[t]	\|\sqrt{\aaa} \utt\|^2_{L^2(\Ltwo)}+  \frac{\delta}{2}\|\nabla \ut(t)\|^2_{\Ltwo}\Big \vert_0^t+\frac{\delta c^2}{2}\|\Delta u(t)\|^2_{\Ltwo} \Big \vert_0^t
	\end{multlined} \\
\lesssim&\, \begin{multlined}[t] \|\aaa_t\|^2_{L^\infty(L^4)} \|\ut\|^2_{L^2(L^4)} + \|\Delta u\|^2_{L^2(L^2)} + \|f\|^2_{L^2(L^2)}+\varepsilon \|\utt\|^2_{L^2(L^2)}+\varepsilon \|\Delta u\|^2_{L^2(L^2)} \\
	- c^2\inttO (\aaa+ 1) \Delta u \utt \dxs
	+ \taua \|u_2\|^2_{L^2} +\|\Delta u_0\|^2_{L^2}. 
	\end{multlined}
	\end{aligned}
\end{equation}
The $\aaa+1$ term on the right we can treat as follows:
\begin{equation}
	\begin{aligned}
	\left| \inttO (\aaa+ 1) \Delta u \utt \dxs\right| \lesssim&\, (\olaaa+1) \|\Delta u\|_{L^2(L^2)}\|\utt\|_{L^2(L^2)} \\
	\lesssim&\, \|\ \Delta u\|^2_{L^2(L^2)} + \|\Delta u\|_{L^2(L^2)}^2 + \varepsilon \|\utt\|_{L^2(L^2)}^2.
	\end{aligned}
\end{equation}
Thus selecting $\varepsilon>0$ small enough and applying Gronwall's inequality leads to the following uniform bound:
\begin{equation}
	\begin{aligned}
	&\begin{multlined}[t]	\|\sqrt{\aaa} \utt\|^2_{L^2(L^2)}+  \|\nabla \ut(t)\|^2_{\Ltwo}+\|\Delta u(t)\|^2_{L^2} 
	\end{multlined} \\
	\leq&\, \begin{multlined}[t] C_{\textup{lin}} \left\{\|\Delta u_0\|^2_{L^2}+\|\nabla u_1\|^2+\taua \|u_2\|^2_{L^2}+\|f\|^2_{L^2(L^2)}\right\}
	\end{multlined}
	\end{aligned}
\end{equation}
a.e.\ in time. Note that the constant has the form
\begin{equation}\label{C_lin}
	C_{\textup{lin}}=C\exp\left\{(1+ \|\aaa_t\|^2_{L^\infty(L^4)})T\right\}
\end{equation}
and tends to $\infty$ as $\delta \searrow 0$, but it is independent of $\tau$. Thus the presence of the strong damping $-\delta \Delta \ut$ in the limiting equation is essential for this testing procedure to work. 
\begin{remark}[Initial data for the equation with Westervelt-type nonlinearities in pressure form]
	If we follow the derivation in Section~\ref{Sec:Modeling} leading to the Westervelt-type equation \eqref{JMGT_West_nonlocal_pressure} in the so-called pressure form with source term given in \eqref{source_Westervelt_type}, we would need to assume the initial data to be zero for the analysis in Section~\ref{Sec:WestType} to hold, as otherwise we cannot have $L^2(0,T)$ regularity of the right-hand side. However, since equation \eqref{GFE_type_eq} and its treatment might be of independent interest (as our analysis shows, \eqref{GFE_type_eq} might be seen as an approximation of the classical damped Westervelt equation in pressure form), we consider it below with general initial conditions and source term.
\end{remark}
We first prove the following existence result for a linearized problem which we intend to later combine with a fixed-point approach. As we are interested in the limiting behavior as $\tau \searrow 0$, we restrict our considerations to $\tau \in (0, \bar{\tau}]$ for some given fixed $\bar{\tau}>0$.
\begin{proposition}\label{Prop:Wellp_GFE_lin}
	Let $T>0$, $\delta>0$, and $\tau \in (0, \bar{\tau}]$. %\vanja{The analysis seems to go through for the Westervelt equation with $\tau=0$ (and even $\bbb=0$), which makes me suspicious since in \cite{kaltenbacher2009global} one needs $u_1 \in \Honetwo$ when using energy arguments. Although this regularity setting agrees exactly with Meyer \& Wilke \cite[Theorem 1.1, $p=2$]{meyer2011optimal}} 
	Let  $\frakKone \in L^1(0,T)$ and let assumption \eqref{eqn:Alikhanov_1} on the kernel $\frakKone$ hold. Furthermore, assume that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone*\tfrakKone=1$. Let the coefficients $\aaa$ satisfy 
	\[
	\aaa \in L^\infty(0,T; L^\infty(\Omega)) \cap W^{1,\infty}(0,T; L^4(\Omega)).
	\]
	 and assume that $\aaa$ does not degenerate so that \eqref{nondeg_aaa} holds. Let $f \in L^2(0,T; L^2(\Omega))$ and
	\begin{equation}
		\begin{aligned}
			(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2) \in \Honetwo \times \Honezero \times \Ltwo.
		\end{aligned}
	\end{equation}
	Then there exists a solution
	% \mostafa{Maybe the fact that $\frakKone\Lconv \uttt \in L^2(0,T;H^{-1}(\Om))$ should be added to the definition of $\calUGFE$ as it justifies the validity of the weak form? I would expect otherwise that we need smoother test functions in time \Vanja{But this follows by the PDE (i.e., bootstrapping) so I do not know if we necessarily have to add it?}}
	\begin{equation} \label{def_calU_GFE}
	u \in \calUGFE = L^\infty(0,T; \Honetwo) \cap W^{1, \infty}(0,T; \Honezero) \cap H^2(0,T; \Ltwo)
	\end{equation} of the following problem:
\begin{comment}
	\begin{equation} \label{IBVP_Westtype_lin}
		\left \{	\begin{aligned}
			&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t+\aaa(x,t) u_{tt}
				-c^2 \bbb(x,t) \Delta u -\delta \Delta \ut=f(x,t),\end{multlined}\\
			&u\vert_{\partial \Omega}=0, \\
			&	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2).
		\end{aligned} \right. 
	\end{equation}
\end{comment}
	\begin{equation} \label{weak_GFE_lin}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	\intTO {\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t v \dxs+\intTO \aaa(x,t) u_{tt} v\dxs
			\\-c^2 \intTO  \Delta u v \dxs 
			+\delta \intTO\nabla \ut \cdot \nabla v \dxs\\ = \intTO f(x,t) v \dxs,\end{multlined}
	\end{aligned} \right. 
\end{equation}
for all $v \in L^2(0,T; \Honezero)$, with $	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2)$ which satisfies the following estimate: 
	\begin{equation}\label{final_est_GFE_lin}
		\begin{aligned}
			\|u\|_{\calUGFE}^2 \lesssim_T \|u_0\|^2_{H^2}+\|u_1\|^2_{H^1} + \tau^a  \|u_2\|^2_{L^2}+ \|f\|_{L^2(L^2)}^2,
		\end{aligned}
	\end{equation}
	where the hidden constant tends to $\infty$ as either $T \rightarrow \infty$ or $\delta \rightarrow \infty$, but does not depend on $\tau.$ 
\end{proposition}
\begin{remark}
For fractional kernels $\frakKone(t)=\frac{1}{\Gamma(1-\alpha)}t^{-\alpha}$, the condition that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone*\tfrakKone=1$, is equivalent to $\alpha>\frac12$; see, for example,~\cite[Ch.\ 6]{jin2021fractional}. 
\end{remark}
\begin{proof}
	We conduct the proof %as in the proof of Proposition~\ref{Prop:Wellp_GFEIII_lin} 
	using a Galerkin semi-discretization in space based on a finite-dimensional subspace $V_n \subset \Honetwo$; see, e.g., \cite[Proposition 5.2]{kaltenbacher2022time} for similar arguments in the analysis of time-fractional wave-like equations. The distinguishing feature of the present Galerkin analysis is that it should be uniform with respect to the relaxation time. By relying on the existence theory for the Volterra integral equations~\cite{gripenberg1990volterra}, we can prove that there is a unique approximate solution $\un \in W^{2, \infty}(0,T; V_n)$. As these arguments are relatively common, we postpone their details to Appendix~\ref{Appendix:Galerkin}.  \\
	\indent Using the estimation techniques outlined at the beginning of this section, we derive the following bound on $\un$:
	\begin{equation} \label{est_discrete_GFE_lin}
		\begin{aligned}
			&\begin{multlined}[t]	\|\sqrt{\aaa} \untt\|^2_{L^2(L^2)}+  \|\nabla \unt(t)\|^2_{\Ltwo}+\|\Delta \un(t)\|^2_{L^2} 
			\end{multlined} \\
			\lesssim_T&\, \begin{multlined}[t] \|\Delta u_0\|^2_{L^2}+\|\nabla u_1\|_{L^2}^2+\taua \|u_2\|^2_{L^2}+\|f\|^2_{L^2(L^2)}. 
			\end{multlined}
		\end{aligned}
	\end{equation}
Below we do not relabel any subsequences. Thanks to this bound that is uniform in $n$, there is a subsequence, such that
	\begin{equation} \label{weak_limits_GFE_1}
	\begin{alignedat}{4} 
		\un &\relbar\joinrel\rightharpoonup u && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honetwo),  \\
		\unt &\relbar\joinrel\rightharpoonup u_t && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honezero),\\
		\untt &\relbar\joinrel\rightharpoonup u_{tt} && \quad \text{ weakly}  &&\text{ in } &&L^2(0,T; \Ltwo).
	\end{alignedat} 
\end{equation} 
We also have the following uniform bound on the leading term:
\begin{equation}
	\begin{aligned}
	&\|	{\tau^a}  \frakKone * (\untt-c^2 \Delta \un)_t\|_{L^2(\Hneg)}\\
	=&\|-\aaa(x,t) \untt
	+c^2  \Delta \un +\delta \Delta \unt+f(x,t)\|_{L^2(\Hneg)} \leq C,
	\end{aligned}
\end{equation}
and thus
\begin{equation}
	\begin{aligned}
		\|	{\tau^a}  \frakKone * \unttt\|_{L^2(\Hneg)}\ \leq  c^2	\|	{\tau^a}  \frakKone * \Delta \unt\|_{L^2(\Hneg)} +C \leq \tilde{C},
	\end{aligned}
\end{equation}
where the constants $C$ and $\tilde{C}$ do not depend neither on $n$ nor on $\tau$. Therefore, {since $\tfrakKone \in L^2(0,T)$}, by Lemma~\ref{Lemma:Caputo_seq_compact}, we have 
\begin{comment} \vanja{We could likely do without this restriction on $\tfrakKone$ if the first term in the equation is understood weakly
		\[
		-\taua\inttO \frakKone * \utt v_t \dxs - \taua \inttO \frakKone(s) u_2 v \dxs
		\] but then it is impossible to test with something useful in the continuous setting}
\end{comment}		
	\begin{equation} \label{weak_limits_GFE_2}
	\begin{alignedat}{4} 
	{\tau^a}  \frakKone * \unttt  &\relbar\joinrel\rightharpoonup 	{\tau^a}  \frakKone * \uttt && \quad \text{ weakly}  &&\text{ in } &&L^2(0,T; \Hneg).
	\end{alignedat} 
\end{equation} 
We can then pass to the limit in the semi-discrete problem in the usual way and show that $u$ solves \eqref{weak_GFE_lin}. \\
\indent By the weak limits in \eqref{weak_limits_GFE_1} and the Aubin--Lions--Simon lemma (see~\cite[Corollary 4]{simon1986compact}), we have
	\begin{equation} \label{weak_limits_GFE_3}
	\begin{alignedat}{4} 
		\un&\longrightarrow u && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Honezero),  \\
		\unt &\longrightarrow u_t && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Ltwo)),
	\end{alignedat} 
\end{equation} 
from which we conclude that $u(0)=u_0$ and $u_t(0)=u_1$. We next show that $u$ also attains the third initial condition. 
Let $v \in C^1([0,T]; \Honezero)$ with $v(T)=v_t(T)=0$. By subtracting the weak forms for $u$ and $\un$, where we integrate by parts in the convolved term, and then passing to the limit,  we obtain
\begin{equation}
	\begin{aligned}
	 &%\taua \inttO (\frakKone * (\un-c^2 \Delta \un))v(0)\dx 
	-\taua \inttO \frakKone(s)(u_2-c^2 \Delta u_0) v \dxs \\
	=&\, 	 \taua \inttO (\frakKone * (\utt-c^2 \Delta u))(0)v(0)\dx 
	-\taua \inttO \frakKone(s)(\utt(0)-c^2 \Delta u_0)v \dxs .
	\end{aligned}
\end{equation}
Noting that $(\frakKone * \Delta u)(0)=0$ gives
\begin{equation}\label{attaining_u2}
	\begin{aligned}
 \taua \inttO (\frakKone * \utt)(0)v(0)\dx 
		-\taua \inttO \frakKone(s)(\utt(0)-u_2)v \dxs =0.
	\end{aligned}
\end{equation}
The first term on the left above is also equal to zero. Indeed, since $\tfrakKone \in L^2(0,T)$, then  from the  bound on 
\begin{equation}
	\begin{aligned}
		\taua \frakKone* \unttt := \tilde{f}^{(n)}
	\end{aligned}
\end{equation}
in $L^2(0,T; H^{-1}(\Omega))$, we obtain a bound on
\begin{equation} \label{Linf_bound_untt}
	\begin{aligned}
		\taua\|\untt\|_{L^\infty(H^{-1})}=&\, \taua\|\un_2 + \tfrakKone*\tilde{f}^{(n)}\|_{L^\infty(H^{-1})} \\
		\lesssim&\,  \|\un_2\|_{H^{-1}} + \|\tfrakKone\|_{L^2}\|\tilde{f}^{(n)}\|_{L^2(H^{-1})}.
	\end{aligned}
\end{equation}
Further,
\begin{equation} \label{Linf_bound_utt}
	\begin{aligned}
		\taua\|\utt\|_{L^\infty(H^{-1})} \leq &\, \taua \liminf_{n \rightarrow \infty}	\|\untt\|_{L^\infty(H^{-1})} \leq C.
	\end{aligned}
\end{equation}
so we conclude that
\[
 \taua \inttO (\frakKone * \utt)(0)v(0)\dx =0.
\] 
Thus, from \eqref{attaining_u2} we have
\[
	-\taua \inttO \frakKone(s)(\utt(0)-u_2)v \dxs=0
\]
for all $v \in C^1([0,T]; \Honezero)$ with $v(T)=v_t(T)=0$. Therefore, (since $\frakKone$ cannot be zero by the assumptions on its resolvent) we obtain $\utt(0)=u_2$. \\
\indent Thus, $u$ is a solution of the initial boundary-value problem. By the weak limits in \eqref{est_discrete_GFE_lin} and weak lower semicontinuity of norms, we conclude that $u$ satisfies stability bound \eqref{final_est_GFE_lin}.
\end{proof}
Note that $	u \in \calUGFE$ implies the following weak continuity in time:
\begin{equation}
	\begin{aligned}
	  u \in C_w([0,T]; \Honetwo), \ \ut \in C_{w}(0,T; \Honezero).
	\end{aligned}
\end{equation}
We next wish to prove that the solution of the problem we have constructed is the only one. \\
\indent To prove uniqueness, we should show that the only solution $u$ of the homogeneous problem (where $f=0$ and $u_0=u_1=u_2$) is $u=0$. However, we are not allowed to test directly with $y=\utt-c^2 \Delta u \in $ in this setting and replicate the previous energy analysis, as $y$ only belongs to $L^2(0,T; L^2(\Om))$. Instead we employ an approach based on considering an adjoint problem, where we adapt the ideas from \cite[Theorem 3, p.\ 573 and 574]{dautray1992evolution} for integer-order equations.
\begin{comment}
\noindent \emph{Uniqueness}. 
We note that by the previous theory
\[
{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t-\delta \Delta \ut= -\aaa(x,t) u_{tt}
+c^2 \bbb(x,t) \Delta u  
\]
and so
\[
{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t-\delta \Delta \ut  \in L^2(0,T; L^2(\Om)).
\]
\gentodo{Likely one needs to adapt the regularization approach from \cite[p.\ 78, Lemma 4.1]{temam2012infinite} to have that
\begin{equation}
	\begin{aligned}
	&({\tau^a}  \frakKone * (\utt^\varepsilon-c^2 \Delta u^\varepsilon)_t-\delta \Delta \ut^\varepsilon, \utt^\varepsilon-c^2 \Delta u^\varepsilon ) \\
	=&\,  ({\tau^a}  \frakKone * (\utt^\varepsilon-c^2 \Delta u^\varepsilon)_t, \utt^\varepsilon-c^2 \Delta u^\varepsilon )+ \frac12 \delta \left\{ \|\nabla \ut^\varepsilon\|^2_{L^2} +c^2 \ddt \|\Delta u^\varepsilon\|^2_{L^2}\right\}
	\end{aligned}
\end{equation}
and then pass to the limit as $\varepsilon \searrow 0$ above to conclude that 
\begin{equation}
	\begin{aligned}
		&({\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t-\delta \Delta \ut, \utt-c^2 \Delta u ) \\
		=&\,  ({\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t, \utt-c^2 \Delta u )+ \frac12 \delta \left\{ \|\nabla \ut\|^2_{L^2} +c^2 \ddt \|\Delta u\|^2_{L^2}\right\}.
	\end{aligned}
\end{equation}
The rest of the arguments can be repeated as before to obtain an energy bound on $u$ and conclude that it is zero. }
\end{comment}

\begin{lemma}
The solution constructed in Proposition~\ref{Prop:Wellp_GFE_lin} is unique. 
\end{lemma}
\begin{proof}
%\noindent \Vanja{\emph{Uniqueness via the adjoint approach}.}\vanja{This is a bit of an unnecessarily complicated proof but I wanted to see if it works. Interestingly, the issues come from the nonlinearity not convolution. Due to the variable coefficient, additional assumptions are needed for the adjoint problem to be solvable. (The assumption  $\bbb=1$ is just to simplify things a bit.) So this proof approach of uniqueness seems more suitable for linear constant coefficient problems. On the other hand, if our analysis is geared towards the nonlinear problem, the additional assumptions will be fulfilled anyway so we could also leave this proof of uniqueness.} We adapt the ideas from \cite[Theorem 3, p.\ 573 and 574]{dautray1992evolution}.
\indent Given $g \in L^2(0,T; L^2(\Omega))$, consider the adjoint problem after time reversal %\gentodo{probably additional assumptions can be avoided by treating $(ap)_{tt}v$ very weakly in time}
\begin{equation}
	\begin{aligned}
	\begin{multlined}[t]	\taua	\intTO (\frakKone* p)_{ttt}(T-t) v(t)\dxt + \intTO (\tilde{\aaa} p_t)_{t}(T-t) v(t)\dxt \\
		- c^2 \intTO \Delta p(T-t) v \dxt - \taua c^2 \intTO (\frakKone*\Delta p)_t(T-t)v(t)\dxt\\
		- \delta \intTO \nabla p_t(T-t) \cdot \nabla v \dxt = \intTO g(T-t) v \dxt,
		\end{multlined}
	\end{aligned}
\end{equation}
for all $v \in L^2(0,T; \Honezero) $, with $(p, p_t, p_{tt}) \vert_{t=0}=(0,0,0)$ and
\[
\tilde{\aaa}=\aaa(T-t).
\] 
Due to homogeneous initial data, we have $(\frakKone*p)_{ttt}=\frakKone*p_{ttt}$ and $(\frakKone*\Delta p)_t=\frakKone*\Delta p_t.$ By Proposition~\ref{Prop:Wellp_GFE_lin}, this problem has a solution $p \in \calUGFE$ with $\taua p_{tt} \in L^\infty(0,T; \Hneg)$. \\
\indent We test it next with $u$ (which is a valid test function since it belongs to $L^2(0,T; \Honezero)$)and use the following integration by parts formula:
\begin{equation} \label{integration_by_parts}
	\begin{aligned}
\int_0^T q_t(T-t)w(t) \dt =\int_0^T q(T-t) w_t(t) \dt- w(T)q(0)+w(0)q(T),
	\end{aligned}
\end{equation}
and the transposition identity:
\begin{equation} \label{transposition_identity}
	\begin{aligned}
	 \int_0^T (\frakKone*q)(T-t) w(t) \dt=\int_0^T (\frakKone*w)(t)q(T-t)\dt.
	\end{aligned}
\end{equation}
By choosing $v=u$ and relying on \eqref{integration_by_parts}, we obtain
\begin{equation}
		\begin{aligned}
	\taua	\intTO (\frakKone* p)_{ttt}(T-t) u(t)\dxt
	 =\,  \taua	\intTO (\frakKone* p)(T-t) \uttt(t)\dxt,
		\end{aligned} 
\end{equation}
where we have also used $(u, \ut, \utt)\vert_{t=0}=(0,0,0)$ and
\begin{equation}
	(\frakKone* p)(0)=0, \quad 	(\frakKone* p)_t(0)=0, \quad (\frakKone* p)_{tt}(0)=0.
\end{equation}
Then,  by identity \eqref{transposition_identity},
\begin{equation}
	\begin{aligned}
		\taua	\intTO (\frakKone* p)_{ttt}(T-t) u(t)\dxt
		=& \,  \taua	\intTO (\frakKone* p)(T-t) \uttt(t)\dxt \\
		=&\,  \taua	\intTO (\frakKone* \uttt)(t) p(T-t)\dxt .
	\end{aligned} 
\end{equation}
Next, by \eqref{integration_by_parts}, 
\begin{equation}
	\begin{aligned}
		\intTO (\tilde{\aaa} p_t)_{t}(T-t) u(t)\dxt =&\, \intTO p(T-t) (\aaa u_{t})_t(t)\dxt. 
	\end{aligned}
\end{equation}
We can treat the other terms in a similar manner to arrive at (with $\aaa(t)=\tilde{\aaa}(T-t)$)
\begin{equation}
	\begin{aligned}
		&\intTO u(t) g(T-t) \dxt\\
		 =&\, \begin{multlined}[t]
			\taua	\intTO (\frakKone* \uttt)(t) p(T-t)\dxt + \intTO (\aaa \ut )_t(t) p(T-t)\dxt \\
		- c^2 \intTO \Delta u(t) p(T-t) \dxt - \taua c^2 \intTO (\frakKone*\Delta \ut)(t)p(T-t)\dxt\\
		- \delta \intTO \nabla \ut(t) \cdot \nabla p(T-t) \dxt
		\end{multlined} \\
	=&\, 0,
	\end{aligned}
\end{equation}
where in the last line we have used the fact that $u$ solves the original (homogeneous) problem. Since $g$ was arbitrary, from here we conclude that $u=0$.
\end{proof}
We next introduce a fixed-point mapping
\begin{equation}
	\begin{aligned}
		T: \calB \ni u^* \mapsto u, 
	\end{aligned}
\end{equation}
where $u$ solves the linear problem given in \eqref{weak_GFE_lin} with the coefficient
\begin{equation}
	\begin{aligned}
		\aaa(u^*) =&\,1+2k_1 u^*
	\end{aligned}
\end{equation}
and $u^*$ is taken from the ball
\begin{equation}
	\begin{aligned}
		\calB =\left \{ u \in \calUGFE:\right.&\, \, \|u\|_{\calUGFE} \leq R,\ %\|2k_1 \nabla u+2k_2 \nabla \ut\|_{L^\infty(L^4)} \leq m, \\&\,  \|k_1 u+k_2u_t\|_{L^\infty(L^\infty)} \leq \frac{1}{2 },\\
		\left	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2) \}, \right.
	\end{aligned}
\end{equation}
where $R>0$ is independent of $\tau$ and will be determined by the upcoming proof. 
\begin{theorem}[Uniform well-posedness of the equation with Westervelt-type nonlinearities] \label{Thm:WellP_GFE} 
	Let $T>0$ and $\tau \in (0, \bar{\tau}]$. Assume that $c$, $\delta>0$ and $k_1 \in \R$. Let assumption \eqref{eqn:Alikhanov_1} on the kernel $\frakKone$ hold. Furthermore, assume that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone * \tfrakKone =1$. Let
	\begin{equation}
		(u_0, u_1, u_2) \in  \Honetwo \times \Honezero \times  \Ltwo
	\end{equation}
and $f \in L^2(0,T; L^2(\Omega))$. There exists $r>0$, independent of $\tau$, such that if
	\begin{equation}\label{smallness_r_Westervelt}
		\|u_0\|^2_{H^2}+\|u_1\|^2_{H^1} + \bar{\tau}^a C(\frakKone) \|u_2\|^2_{L^2}+ \|f\|^2_{L^2(L^2)} \leq r^2,
	\end{equation}
	then there is a unique solution $u \in \calB$ of the nonlinear problem
\begin{comment}
	\begin{equation} \label{IBVP_Westtype_nonlin}
		\left \{	\begin{aligned}
			&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t+\aaa(u) u_{tt}
				-c^2  \Delta u  -\delta   \Delta \ut +\calN(\ut)=0,\end{multlined}\\
			&u\vert_{\partial \Omega}=0, \\
			&	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2).
		\end{aligned} \right. 
	\end{equation}
\end{comment}
	\begin{equation} \label{weak_GFE}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	\intTO \taua  \frakKone * (\utt-c^2 \Delta u)_t v \dxs+\intTO (\aaa(u) u_{t})_t v\dxs
			\\-c^2 \intTO  \Delta u v \dxs 
			+\delta \intTO\nabla \ut \cdot \nabla v \dxs=\intTO f v \dxs,\end{multlined}
	\end{aligned} \right. 
\end{equation}
for all $v \in L^2(0,T; \Honezero)$, with $	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2)$. The solution depends continuously on the data with respect to $\|\cdot\|_{\calUGFE}$.
\end{theorem}
\begin{proof}
We check that the conditions of the Banach fixed-point theorem are satisfied. \\[2mm]
	\noindent \emph{Self-mapping}.  Let $u^* \in \calB$. Since then $u^* \in \calUGFE$, the smoothness assumptions on $\aaa$ in Proposition~\ref{Prop:Wellp_GFE_lin} are satisfied and the non-degeneracy assumption on $\aaa$ is fulfilled by reducing $R>0$ since
	\[
	\|2k_1 u^*\|_{L^\infty(L^\infty)} \leq C(\Omega, T)|k_1| R.
	\]
	Further, we have the bound
	\begin{equation}
		\|\aaa_t\|_{L^\infty(L^4)} \lesssim 	\|u^*_t\|_{L^\infty(H^1)} \lesssim R. 
	\end{equation}
By employing Proposition~\ref{Prop:Wellp_GFE_lin}, we obtain 
	\begin{equation}
		\begin{aligned}
			\|u\|_{\calUGFE} 
			\leq\,
			C_{\textup{lin}}(\|u_0\|^2_{H^2}+\|u_1\|^2_{H^1} + \tau^a C(\frakKone) \| u_2\|^2_{L^2}+ \|f\|_{L^{2}(L^2)}^2).
		\end{aligned}
	\end{equation}
Thus,
	\begin{equation}
		\begin{aligned}
			\|u\|_{\calUGFE} 
			\leq&\, C\exp((1+R)T)(r^2+CR^4)
		\end{aligned}
	\end{equation}
and $u \in \calB$ for sufficiently small $r$ and the radius $R$ (independently of $\tau$). \\
	
	\noindent \emph{Strict contractivity}. Let $T u^{*} =u$ and $T v^*=v$. We denote $\phi=u-v$ and $\phi^*= u^*-v^*$. Then $\phi$ is a solution of  
	\begin{equation}
		\begin{aligned}
			\begin{multlined}[t]	{\tau^a}  \frakKone *( \phi_{tt}-c^2 \Delta \phi)_t+(\aaa(u^*) \phi_{t})_t
				-c^2  \Delta \phi
				-   \delta   \Delta \phi_{tt}\end{multlined}
			=\, -2k_1 (\phi^* v_{t})_t.
		\end{aligned}
	\end{equation}
This has the form of the linear problem with $f= -2k_1 (\phi^* v_{t})_t$. Thus bound \eqref{final_est_GFE_lin}  implies 
\begin{equation}
	\begin{aligned}
	\| \phi\|_{\calUGFE} \lesssim&\, \|-2k_1 \phi^* v_{tt} -2k_1 \phi^*_t v_t\|_{L^2(L^2)} \\
	\lesssim&\, \|\phi^*\|_{L^\infty(L^\infty)} \|v_{tt}\|_{L^2(L^2)} + \|\phi^*_t \|_{L^\infty(L^4)}\|v_t\|_{L^2(L^4)} 
		\lesssim\, R \|\phi^*\|_{\calUGFE},
	\end{aligned}
\end{equation}
from which we obtain strict contractivity for small enough $R$.
\end{proof}
\subsection{Weak singular limit for the vanishing relaxation time}\label{Subsec:Weaklim_tau_GFE} Let $\tau \in (0, \bar{\tau}]$. Consider the following initial boundary-value problem:
\begin{equation} \label{IBVP_GFE_tau}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t+(\aaa(u^\tau) \ut^\tau)_t
			-c^2 \Delta u^\tau 
		-\delta   \Delta \ut^\tau=f ,\end{multlined}\\
		&u^\tau\vert_{\partial \Omega}=0, \\
		&	(u^\tau, \ut^\tau, \utt^\tau)\vert_{t=0} =(u_0, u_1, u_2).
	\end{aligned} \right. 
\end{equation}
From the previous analysis, under the assumptions of Theorem~\ref{Thm:WellP_GFE}, we have the following uniform bounds with respect to the thermal relaxation time $\tau$:
\begin{equation}\label{uniform_bounds_tau_West}
	\left \{	\begin{aligned}
		&u^\tau \ \text{is bounded in } L^\infty(0,T; \Honetwo), \\
		&\ut^\tau  \ \text{is bounded in } L^\infty(0,T; \Honezero), \\
		&\utt^\tau  \ \text{is bounded in } L^2(0,T; \Ltwo). 
	\end{aligned} \right.
\end{equation}
Additionally, since $\tfrakKone \in L^2(0,T)$, $\taua \utt^\tau$ is uniformly bounded in $L^2(0,T; \Hneg)$. Therefore, by \eqref{uniform_bounds_tau_West}, there exists a subsequence, not relabeled, such that 
\begin{equation} \label{weak_limits_tau_GFE_1}
	\begin{alignedat}{4} 
		u^\tau&\relbar\joinrel\rightharpoonup u && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honetwo),  \\
		\ut^\tau &\relbar\joinrel\rightharpoonup u_t && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honezero),\\
		\utt^\tau &\relbar\joinrel\rightharpoonup u_{tt} && \quad \text{ weakly}  &&\text{ in } &&L^2(0,T; \Ltwo).
	\end{alignedat} 
\end{equation} 
By the Aubin--Lions--Simon lemma, this further implies
\begin{equation} \label{weak_limits_tau_GFE_2}
	\begin{alignedat}{4} 
		u^\tau&\longrightarrow u && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Honezero),  \\
		\ut^\tau &\longrightarrow u_t && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Ltwo)).
	\end{alignedat} 
\end{equation} 
Additionally, similarly to before,
\begin{equation}
	\begin{aligned}
		&\|	{\tau^a}  \frakKone * (\utt^\tau-c^2 \Delta u^\tau)_t\|_{L^2(\Hneg)}\\
		=&\|-\aaa(x,t) \utt^\tau
		+c^2 \Delta u^\tau +\delta \Delta \ut^\tau+f(x,t)\|_{L^2(\Hneg)} \leq C,
	\end{aligned}
\end{equation}
and thus we also have a bound on
\begin{comment}
\begin{equation}
	\begin{aligned}
		\|	{\tau^a}  \frakKone * \uttt^\tau\|_{L^2(\Hneg)}\ \leq  c^2	\|	{\tau^a}  \frakKone * \Delta \ut^\tau\|_{L^2(\Hneg)} +C \leq \tilde{C},
	\end{aligned}
\end{equation}
where the constants $C$ and $\tilde{C}$ do not depend on  $\tau$. 
\end{comment}
\begin{equation} \label{Linf_bound_utau_tt}
\begin{aligned}
\taua\|\utt^\tau\|_{L^\infty(H^{-1})}=&\, \taua\|u_2 + \tfrakKone*\left\{-\aaa(x,t) \utt^\tau
+c^2 \Delta u^\tau +\delta \Delta \ut^\tau+f(x,t)\right\}\|_{L^\infty(H^{-1})} \\
\lesssim&\,  \|u_2\|_{H^{-1}} + \|\tfrakKone\|_{L^2}C.
\end{aligned}
\end{equation}
Let $v \in C^\infty([0,T]; C_0^\infty(\Omega))$ with $v(T)=0$. We have with $\bar{u}=u-u^\tau$:
\begin{equation}\label{weak_limit_baru}
	\begin{aligned}
		&\begin{multlined}[t] \intTO (\aaa(u) \ut)_t v \dxs+ c^2 \intTO  \Delta u v \dxs + \delta \intTO  \nabla \ut \cdot \nabla v \dxs\\
			-\intTO f v \dxs \end{multlined}\\
		=&	\begin{multlined}[t]  \intTO ( \aaa(u)\bar{u}_{t})_t v \dxs+ c^2 \intTO  \Delta \bar{u} v \dxs+ \delta \intTO  \nabla \bar{u}_{t} \cdot \nabla v \dxs \\
			- \intTO  \taua \frakKone * (\utt^\tau -c^2 \Delta u^\tau)_t v \dxs 
			+2k_1\intTO (\bar{u}\ut^\tau)_t v \dxs.  \end{multlined}
	\end{aligned}
\end{equation}
We wish to prove that the right-hand side tends to zero as $\tau \searrow 0$. To this end, we exploit  the established weak convergence. By relying on \eqref{weak_limits_tau_GFE_1} and the equivalence of norms $\|\cdot\|_{L^2}$ and $\|\sqrt{a} \cdot\|_{L^2}$, we conclude that 
\begin{equation} 
	\begin{alignedat}{4} 
		\aaa(u) \utt^\tau &\relbar\joinrel\rightharpoonup 	\aaa(u) \utt && \quad \text{ weakly}  &&\text{ in } &&L^2(0,T; \Ltwo).
	\end{alignedat} 
\end{equation} 
Further,
\begin{equation}
\intTO  (\aaa(u))_t\bar{u}_t v \dxs = 2k_1 \intTO  u_t \bar{u}_t v \dxs \lesssim  \|\ut\|_{L^2(L^4)}\|\bar{u}_t\|_{L^\infty(L^2)}\|v\|_{L^2(L^4)},
\end{equation}
which tends to zero by \eqref{weak_limits_tau_GFE_2}. Thus 
\begin{equation}
	\begin{aligned}
		\intTO  (\aaa(u)\bar{u}_{t})_t v \dxs+ c^2 \intTO  \Delta \bar{u} v \dxs + \delta \intTO  \nabla \bar{u}_{t} \cdot \nabla v \dxs  \rightarrow  0 \quad \text{as } \tau \searrow 0.
	\end{aligned}
\end{equation}
We also have
\begin{equation}
	\begin{aligned}
		-2k_1\intTO \bar{u} \utt^\tau v \dxs \lesssim \|\bar{u}\|_{L^\infty(L^4)} \|\utt^\tau\|_{L^2(L^2)} \|v\|_{L^2(L^4)}\rightarrow 0,	
	\end{aligned}
\end{equation}
thanks to \eqref{weak_limits_tau_GFE_2}.  It remains to discuss the convolution term. Since $v(T)=0$, integration by parts yields
\begin{equation}\label{conv_term}
\begin{aligned}
&-\intTO \taua \frakKone*\uttt^\tau v \dxs\\
=&\, -\intTO \taua (\frakKone*\utt^\tau)_t v\dxs + \inttO \taua \frakKone(s)u_2 v \dxs  \\
%=&\, \begin{aligned}[t] \taua  \left\{-\intO(\frakKone*\utt^\tau)(T) v(T) \dx+{\intTO(\frakKone*\utt^\tau)(0) v(0) \dx}+\intTO  \frakKone*\utt^\tau  v_t \dxs \right. \\ \left.+ \inttO  \frakKone(s)u_2 v\dxs\right\}.
	=&\, \begin{multlined}[t] \taua  \left\{\intTO  \frakKone*\utt^\tau  v_t \dxs \right. \left.+ \inttO  \frakKone(s)u_2 v\dxs\right\},
\end{multlined}
\end{aligned}
\end{equation}
where we have also used that, since $\taua \utt^\tau \in L^\infty(0,T; \Hneg)$, $(\frakKone*\taua \utt^\tau)(0) =0$. As the terms in the bracket are uniformly bounded:
\begin{equation}
\begin{aligned}
&\intTO  \frakKone*\utt^\tau  v_t \dxs+ \inttO  \frakKone(s)u_2 v\dxs \\
\lesssim&\, \|\frakKone\|_{L^1(0,T)} \|\utt^\tau\|_{L^2(L^2)}\|v_t\|_{L^2(L^2)}+ \|\frakKone\|_{L^1(0,T)} \|u_2\|_{L^2(\Omega)}\|v\|_{L^1(L^2)},
\end{aligned}
\end{equation}
the convolution term \eqref{conv_term} also converges to zero as $\tau \searrow 0$.  Similarly,
\[
- \intTO  \taua c^2 \frakKone * \Delta u^\tau_t v \dxs  \rightarrow 0.
\]
Therefore, the right-hand side of \eqref{weak_limit_baru} tends to zero as $\tau \searrow 0$ and we thus conclude that $u$ satisfies the limiting Westervelt equation. The attainment of initial conditions $(u_1, u_2)$ follows by \eqref{weak_limits_tau_GFE_2}. \\
\indent Note that the limiting problem with $\tau=0$ is  known to be well-posed with $f=0$; %in $ \calUGFE \, \cap H^1(0,T; \Honetwo)$ 
see \cite[Theorem 1.1]{meyer2011optimal}. The uniqueness of solutions in a general setting can be obtained by testing with, for example $\ut$. Thus by a subsequence-subsequence argument (see, e.g., \cite[Ch.\ 3]{zeidler2012applied}) and the uniqueness of solutions to the limiting problem, we conclude that the whole sequence converges, thus arriving at the following result.
\begin{proposition}[Limiting weak behavior of equations with Westevelt-type nonlinearities] \label{Prop:WeakLim_West}
	Let $T>0$ and $\tau \in (0, \bar{\tau}]$. Let assumption \eqref{eqn:Alikhanov_1} on the kernel $\frakKone \in L^1(0,T)$ hold. Furthermore, assume that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone * \tfrakKone =1$. Let
\begin{equation}
	(u_0, u_1, u_2) \in  \Honetwo \times \Honezero \times  \Ltwo
\end{equation}
and $f \in L^2(0,T; L^2(\Omega))$ with
\begin{equation}
	\|u_0\|^2_{H^2}+\|u_1\|^2_{H^1} + \bar{\tau}^a C(\frakKone) \|u_2\|^2_{L^2}+\|f\|^2_{L^2(L^2)} \leq r^2,
\end{equation} 
with $r>0$ chosen according to Theorem~\ref{Thm:WellP_GFE}. Then the family $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ of solutions to
	\begin{equation} \label{weak_GFE_tau}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	\taua \intTO  \frakKone * (\utt^\tau-c^2 \Delta u^\tau)_t v \dxs+\intTO (\aaa(u^\tau) u^\tau_{t})_t v\dxs
			\\-c^2 \intTO \Delta u^\tau v \dxs 
			+\delta \intTO\nabla \ut^\tau \cdot \nabla v \dxs= \intTO f  \dxs,\end{multlined} \\
	&	\text{for all }\ v \in L^2(0,T; \Honezero), \, \text{with} \ (u^\tau, u^\tau_t, u^\tau_{tt})\vert_{t=0} =(u_0, u_1, u_2)
	\end{aligned} \right. 
\end{equation}
converges weakly in the sense of \eqref{weak_limits_tau_GFE_1} to the solution $u \in \calUGFE \, \cap H^1(0,T; \Honetwo)$ of the Westervelt equation in pressure form: 
	\begin{equation} \label{weak_Westervelt}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	\intTO (\aaa(u) \ut)_t v\dxs
			-c^2 \intTO \Delta u v \dxs  
		-\delta \intTO\Delta \ut  v \dxs\\= \intTO f v \dxs,\end{multlined}\\
	&\text{for all}\ v \in L^2(0,T; \Ltwo), \ \text{with} \ (u, \ut)\vert_{t=0} =(u_0, u_1).
	\end{aligned} \right. 
\end{equation}
\end{proposition}
As a by-product of the limiting analysis, we also obtain solvability of the Westervelt equation in pressure form for (small) initial data in $\Honetwo \times \Honezero$ and source term in $L^2(0,T; L^2(\Omega))$.\vanja{It's not clear to me if we need to enforce for the Westervelt equation the assumption $\utt(0) \in \Ltwo$ (which would mean initial data practically in $\Honetwo \times \Honetwo$). Our discussion in \cite{kaltenbacher2019jordan} suggests that we should. We have the smallness condition \eqref{smallness_r_Westervelt} so we need smallness of $u_2$ but we lose this condition in the limit so how do we get $u_2=\utt(0)$}
\subsection{Strong convergence for the vanishing relaxation time} \label{Subsec:Stronglim_tau_GFEIII} We next wish to prove that the family $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ in fact converges strongly in a suitable norm. To this end, we note that the difference $\bar{u}=u-u^\tau$ weakly solves
\begin{equation} \label{ibvp_diff_u}
	\begin{aligned}
(\aaa(u)\bar{u}_{t})_t-c^2\Delta \bar{u} 
			-\delta   \Delta \bar{u}_t=- 2k_1 (\bar{u}\ut^\tau)_t +	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t 
	\end{aligned}
\end{equation}
with homogeneous data. Having in mind convergence in the standard energy norm (that is, in the space $W^{1,\infty}(0,T; L^2(\Omega)) \cap L^\infty(0,T; \Honezero)$), we could try to test this difference equation with $\bar{u}_t.$ However, the issue arises with the convolution term on the right since
\begin{equation}
	\begin{aligned}
		&-\inttO \taua \frakKone*\uttt^\tau \bar{u}_t \dxs\\
		=&\, -\inttO \taua (\frakKone*\utt^\tau)_t \bar{u}_t \dxs + \inttO \taua \frakKone(s)u_2 \bar{u}_t\dxs  \\
		=&\, \begin{multlined}[t] \taua  \left\{-{\intO(\frakKone*\utt^\tau)(t) \bar{u}_t(t) \dx}+\inttO  \frakKone*\utt^\tau  \bar{u}_{tt}\dxs \right. \left.+ \inttO  \frakKone(s)u_2 \bar{u}_t \dxs\right\}
		\end{multlined}
	\end{aligned}
\end{equation}
and we only have a uniform bound on $\taua \|\frakKone*\uttt^\tau\|_{L^2(H^{-1})}$ and $\taua \|\utt^\tau\|_{L^\infty(L^2)}$ from the previous analysis but not their convergence to zero.
\begin{comment}
\vanja{We have
	\begin{equation}
	u_{tt}^\tau \relbar\joinrel\rightharpoonup \utt  \quad \text{ weakly in} \quad  L^2(0,T; \Ltwo)
	\end{equation} 
	and thus
	%\begin{equation}
	%	\taua u_{tt}^\tau \relbar\joinrel\rightharpoonup 0 \quad \text{ weakly in} \quad  L^2(0,T; \Ltwo).
	%\end{equation}
	%and 
	\begin{equation}
	\taua \frakKone*u_{tt}^\tau \relbar\joinrel\rightharpoonup 0 \quad \text{ weakly in} \quad  L^2(0,T; \Hneg).
	\end{equation}  
	On the other hand, $	\taua \frakKone*u_{tt}^\tau $ is uniformly bounded in $L^\infty(0,T; \Hneg)$ so there is a subsequence such that
	\begin{equation}
	\taua \frakKone*u_{tt}^\tau \relbar\joinrel\rightharpoonup ? \quad \text{ weakly-$*$ in} \quad  L^\infty(0,T; \Hneg).
	\end{equation}
	By the uniqueness of weak limits in $ L^2(0,T; \Hneg)$, we obtain that the limit above is zero. But we do not have a.e. convergence} \\
\end{comment}
\begin{comment}
 by adapting the ideas from \cite[p.\ 580, Ch.\ XVIII]{dautray1992evolution}, where the convergence of parabolic approximations to linear wave equations has been considered.  We have that $u$ and $u^\tau$ satisfy the following identities (after testing the respective equations with $u_t$ and $u_t^\tau$):
\begin{equation}\label{energy_identity_u_GFE}
	\begin{aligned}
		&\frac12  \|\ut(t)\|^2_{L^2}+\frac{c^2}{2} \|\nabla u(t)\|^2_{L^2}+\frac{\delta}{2}\intt \|\nabla u_t\|^2_{L^2}\ds \\
		= &\,	\begin{multlined}[t] N[u](t)+	\frac12  \|u_1\|^2_{L^2}+\frac12  \|\nabla u_0\|^2_{L^2}+\intt \|f\|^2_{L^2}\ds	\end{multlined}
	\end{aligned}
\end{equation}
with the nonlinear terms grouped into
\begin{equation}
	\begin{aligned}
	N[u](t)=
			-\inttO 2k_1 u u_{tt}u_t \dxs -\inttO \calN(\ut) u_t \dxs,
	\end{aligned}
\end{equation}
and
\begin{equation}
	\begin{aligned}
		&	\begin{multlined}[t]	\frac12  \|\ut^\tau(t)\|^2_{L^2}+\frac{c^2}{2}  \|\nabla u^\tau(t)\|^2_{L^2} +\frac{\delta}{2}\intt \|\nabla u^\tau_t\|^2_{L^2}\ds	\end{multlined}\\
		= &\,	\begin{multlined}[t]  N[u^\tau](t)
			+ \frac12  \|u_1\|^2_{L^2}+\frac12  \|\nabla u_0(t)\|^2_{L^2}  +\intt \|f\|^2_{L^2}\ds\\ -\inttO \taua \frakKone*(\utt^\tau-c^2 \Delta u^\tau)_t \ut^\tau \dxs.
		\end{multlined}
	\end{aligned}
\end{equation}
Adding the two identities yields
\begin{equation} \label{strong_conv_identity}
	\begin{aligned}
		&	\begin{multlined}[t]	\frac12 \|\bar{u}_t(t)\|^2_{L^2}+\frac{c^2}{2} \|\nabla \bar{u}(t)\|^2_{L^2}+\frac{\delta}{2}\intt \|\nabla \bar{u}_t\|^2_{L^2}\ds	\end{multlined} \\
		= &\, 	\begin{multlined}[t] 
			Z_\tau(t) -\inttO \taua \frakKone*(\utt^\tau -c^2 \Delta u^\tau)_t \ut^\tau \dxs,
		\end{multlined}
	\end{aligned}
\end{equation}
where
\begin{equation}
	\begin{aligned}
		Z_\tau(t)
		= &\, 	\begin{multlined}[t] N[u](t)+ N[u^\tau](t)- (\ut(t), \ut^\tau(t))_{L^2} - c^2(\nabla u(t),  \nabla u^\tau(t))_{L^2}  \\  - \delta  \int_0^t (\nabla \ut, \nabla \ut^\tau)_{L^2}  \ds 
			+	\|u_1\|^2_{L^2}+  \|\nabla u_0\|^2_{L^2}+2\intt \|f\|^2_{L^2}\ds.
		\end{multlined}
	\end{aligned}
\end{equation}
We wish to show that the right-hand side of \eqref{strong_conv_identity} tends to zero as $\tau \searrow 0$ using the weak convergence results established in \eqref{weak_limits_tau_GFE_1}.  We first consider the $Z_\tau$ term. 
By \eqref{weak_limits_tau_GFE_2}, we find that
\begin{equation} \label{weak_limits_pointwise}
	\begin{alignedat}{4} 
		u_t^\tau(t)&\longrightarrow  u(t)&& \quad \text{ strongly}  &&\text{ in } &&\Ltwo,  \\
		\nabla 	u^\tau (t) &\longrightarrow \nabla u(t)&& \quad \text{ strongly}  &&\text{ in } && \Ltwo,
	\end{alignedat} 
\end{equation} 
as $\tau \searrow 0$. Therefore, we have 
\begin{equation}
	\begin{aligned}
		&\, 	\begin{multlined}[t] - (\ut(t), \ut^\tau(t))_{L^2} - c^2(\nabla u(t),  \nabla u^\tau(t))_{L^2}  
			+	\|u_1\|^2_{L^2}+  \|\nabla u_0\|^2_{L^2} \\ +2\intt \|f\|^2_{L^2}\ds- \delta  \int_0^t (\nabla \ut, \nabla \ut^\tau)_{L^2}  \ds 
		\end{multlined} \\
		\rightarrow&\,  \begin{multlined}[t] - (\ut(t), \ut(t))_{L^2} - c^2(\nabla u(t),  \nabla u(t))_{L^2}  
			+	\|u_1\|^2_{L^2}+  \|\nabla u_0\|^2_{L^2} \\+2\intt \|f\|^2_{L^2}\ds- \delta  \int_0^t (\nabla \ut, \nabla \ut)_{L^2}  \ds .	\end{multlined}  
	\end{aligned}
\end{equation}
Furthermore, as $\tau \searrow 0$ 
\begin{equation}
	N[u](t)+ N[u^\tau]
	\rightarrow 2 N[u](\tau).
\end{equation}
To see this, we note that
\begin{equation}
	\begin{aligned}
		N[u](t)-N[u^\tau](t)=&\, \begin{multlined}[t]
			-2k_1\inttO \left\{\bar{u}\ut^\tau \utt^\tau + u\bar{u}_t \utt^\tau +u\ut \bar{u}_{tt} \right\}\dxs \\
			-2k_4 \inttO \bar{u}_t ((u^\tau_t)^2 + u_t u^\tau + u_t^2) \dxs.
		\end{multlined} 
	\end{aligned}
\end{equation}
By \eqref{weak_limits_tau_GFE_1} and \eqref{weak_limits_tau_GFE_2}, it follows that the right-hand side tends to zero. \gentodo{check} \\
\indent The two limits combined with \eqref{energy_identity_u_GFE} guarantee that for all $t\in [0,T]$, $|Z_\tau(t)| \rightarrow 0 $ as $\tau \searrow 0$.  We next consider the remaining convolution term on the right-hand side of \eqref{strong_conv_identity}. We have \gentodo{the red term does not work out} 
\begin{equation}
	\begin{aligned}
		&-\inttO \taua \frakKone*\uttt^\tau \ut^\tau \dxs\\
		=&\, -\inttO \taua (\frakKone*\utt^\tau)_t \ut^\tau \dxs + \inttO \taua \frakKone(s)u_2 \ut^\tau \dxs  \\
		=&\, \begin{multlined}[t] \taua  \left\{-\textcolor{red}{\intO(\frakKone*\utt^\tau)(t) \ut^\tau(t) \dx}+{\intO(\frakKone*\utt^\tau)(0) u_1 \dx}+\inttO  \frakKone*\utt^\tau  \utt^\tau \dxs \right. \\ \left.+ \inttO  \frakKone(s)u_2 \ut^\tau \dxs\right\}.
		\end{multlined}
	\end{aligned}
\end{equation}
{\color{red} Can one combine $\utt^\tau \relbar\joinrel\rightharpoonup u_{tt}$ weakly in $L^2(0,T; \Ltwo)$ and $\taua \frakKone*\utt^\tau$ uniformly bounded in $L^\infty(0,T; \Hneg)$ to show that the red term goes to zero? We have
\begin{equation}
		u_{tt}^\tau \relbar\joinrel\rightharpoonup \utt  \quad \text{ weakly in} \quad  L^2(0,T; \Ltwo)
\end{equation} 
and thus
%\begin{equation}
%	\taua u_{tt}^\tau \relbar\joinrel\rightharpoonup 0 \quad \text{ weakly in} \quad  L^2(0,T; \Ltwo).
%\end{equation}
%and 
\begin{equation}
	\taua \frakKone*u_{tt}^\tau \relbar\joinrel\rightharpoonup 0 \quad \text{ weakly in} \quad  L^2(0,T; \Hneg).
\end{equation}  
On the other hand, $	\taua \frakKone*u_{tt}^\tau $ is uniformly bounded in $L^\infty(0,T; \Hneg)$ so there is a subsequence such that
\begin{equation}
	\taua \frakKone*u_{tt}^\tau \relbar\joinrel\rightharpoonup ? \quad \text{ weakly-$*$ in} \quad  L^\infty(0,T; \Hneg).
\end{equation}
By the uniqueness of weak limits in $ L^2(0,T; \Hneg)$, we obtain that the limit above is zero. But we do not have a.e. convergence } \\
We have as before 
	\[
	(\frakKone*\taua \utt^\tau)(0) =0.
	\]
The remaining terms in the bracket can be uniformly bounded as follows: 
\begin{equation}
	\begin{aligned}
		&\left |\inttO  \frakKone*\utt^\tau  \utt^\tau \dxs + \inttO  \frakKone(s)u_2 \ut^\tau \dxs \right| \\
		\lesssim&\, \begin{multlined}[t]\| \|\frakKone\|_{L^1(0,T)} \|\utt^\tau\|_{L^2(L^2)}^2+\|\frakKone\|_{L^1(0,T)}\|u_2\|_{L^2}\|\ut^\tau\|_{L^\infty(L^2)}. \end{multlined}
	\end{aligned}
\end{equation}
Additionally, 
\begin{equation}
	\begin{aligned}
		\left|	\inttO \taua c^2 \frakKone* \Delta \ut^\tau \ut^\tau \dxs \right| \leq \taua \|\frakKone\|_{L^1(0,T)} \|\nabla \ut^\tau\|^2_{L^2(L^2)}.
	\end{aligned}
\end{equation}
\begin{comment}
Altogether, we conclude that
\begin{equation} 
	\begin{aligned}
		&	\begin{multlined}[t]	\frac12 \|\bar{u}_t(t)\|^2_{L^2}+\frac{c^2}{2} \|\nabla \bar{u}(t)\|^2_{L^2}+\frac{\delta}{2}\intt \|\nabla \bar{u}_t\|^2_{L^2}\ds	\end{multlined} \rightarrow 0 \quad \text{as} \ \tau \searrow 0.
	\end{aligned}
\end{equation}
\end{comment}

\begin{comment}
\subsection{An attempt to get a bound on $\|\utt \|_{L^\infty(L^2)}$} We assume also
 \begin{equation}\label{coercivity_frakKone}
	\int_0^{t'} \int_0^t\frakKone(t-s) y(s)\ds \,y(t)\dt \geq \tilde{C}_{\frakKone} \|y\|^2_{H^{-\gamma}(0,t)}, \quad y ?. 
\end{equation}
We then additionally test in the semi-discrete setting with $(\untt-c^2 \Delta \un)_t$, which at first results in
\begin{equation}
	\begin{aligned}
	&\taua \|\unttt-c^2 \Delta \unt\|^2_{H^{-\gamma}(L^2)}+	\intt	( \aaa \untt-c^2\bbb\Delta \un - \delta \Delta \unt, \unttt-c^2 \Delta \unt)_{L^2} \ds\\
	 \lesssim&\, \intt (f, (\untt-c^2 \Delta \un)_t)_{L^2}\ds.
	\end{aligned}
\end{equation}
From here,
\begin{equation}
	\begin{aligned}
		&\begin{multlined}[t] \taua \|\unttt-c^2 \Delta \unt\|^2_{H^{-\gamma}(L^2)} \\
			+\frac12	\|\sqrt{\aaa} \untt(s)\|^2_{L^2} \big \vert_0^t+ \frac{c^2}{2}\|\sqrt{\bbb}\Delta \un(s)\|^2_{L^2(L^2)}+\delta c^2 \intt \|\Delta \unt\|^2_{L^2}\ds  \end{multlined} \\
		\lesssim&\, \begin{multlined}[t]\frac12 \inttO \aaa_t (\untt)^2 \dxs-\frac{c^2}{2} \inttO \bbb_t |\Delta \un|^2 \dxs
			+ c^2\inttO \aaa  \untt \Delta \unt \\
			+ \inttO (c^2 \bbb \Delta \un\Vanja{+\delta \Delta \unt)  \unttt \dxs} +  (f, (\untt-c^2 \Delta \un)_t)_{L^2}\ds \big \vert_0^t \\+\intt (f_t, \untt-c^2 \Delta \un)_{L^2}\ds.  \end{multlined}
	\end{aligned}
\end{equation}
\Vanja{One might assume $\delta=O(\sqrt{\taua})$ to treat the blue term, but we would need more regularity in time of $\Delta \unt$}
  \subsection{Discussion of other equations} {Along the same lines,} 
  for other (linear) equations, we could express $\frakKtwo= \mathfrak{r} * \frakKone$ as in \cite{meliani2023}, write the equations as \[\taua \frakKone *(\utt-c^2\Delta u-\frac{\rt^b \delta}{\taua} \mathfrak{r} *\Delta \ut)_t+ \utt-c^2\Delta u =f, \] and test with $y= \utt-c^2\Delta u-\frac{\rt^b \delta}{\taua} \mathfrak{r} *\Delta \ut$ or $y_t$.  For $\rt^b  \delta / \taua =$const.\ (to get to a uniform bound), testing with $y$ would result in (up to initial conditions on the rhs)
  \begin{equation}
  	\begin{aligned}
  	& \begin{multlined}[t]	\|\utt-c^2 \Delta u\|^2_{L^2(L^2)} +\frac{\rt^b \delta}{\tau} \inttO (\mathfrak{r} * \nabla \ut) \cdot \nabla \utt \dxs \\
  		+ \frac{\rt^b \delta}{\taua} c^2 \inttO (\mathfrak{r} * \Delta \ut) \Delta u \dxs 
  		\end{multlined}\\
  	\lesssim&\, \begin{multlined}[t] \|f\|^2_{L^2(L^2)} +\varepsilon \|\utt-c^2 \Delta u\|^2_{L^2(L^2)} 
  		+  \frac{\rt^b \delta}{\taua}\inttO f (\mathfrak{r} * \Delta \ut) \dxs.
  		\end{multlined}
  	\end{aligned}
\end{equation}
If $\mathfrak{r}$ satisfies \eqref{eqn:boundedness_frakK}, \eqref{eqn:Alikhanov_1}, then 
  \begin{equation}
	\begin{aligned}
&\frac{\rt^b \delta}{\taua} \inttO (\mathfrak{r} * \nabla \ut) \cdot \nabla \utt \dxs 
+ \frac{\rt^b \delta}{\taua} c^2 \inttO (\mathfrak{r} * \Delta \ut) \Delta u \dxs  \\
\geq&\, -\frac{\rt^b \delta}{\taua} C_\gamma \|\nabla \utt\|^2_{H^{-\gamma}(L^2)} - \frac{\rt^b \delta}{\taua} c^2 C_{\mathfrak{r}} \|\Delta u_0\|^2_{L^2} ,
  	\end{aligned}
\end{equation}
which does not seem possible to control. The estimates do work if $\delta=0$ at least.  \\
\subsubsection{Strong convergence in the $L^\infty(0,T; L^2(\Omega)) \cap L^2(0,T; \Honezero)$ norm for the vanishing relaxation time} 
\end{comment}
We adapt here instead the ideas from \cite[Section TBD]{meliani2023} to obtain strong convergence in a weaker norm than the energy one. To this end, for $t' \in (0,T)$, we use the following test function (see also \cite{evans2010partial} and \cite{kaltenbacher2021determining} for similar ideas employed when proving uniqueness of solutions):
\begin{equation}\label{test_function}
\begin{aligned}
v(t)= \begin{cases}
\int_t^{t'} \bar{u}(s) \ds \quad &\text{if} \ 0 \leq t \leq t', \\[1mm]
0 \qquad &\text{if} \  t' \leq t \leq T,
\end{cases}
\end{aligned}
\end{equation}
where $\bar{u}=u^\tau-u$. Then we conveniently have $v_t= -\bar{u}$ if $ 0 \leq t \leq t'$, otherwise $v_t=0$. Further, given a Hilbert space $H$, the following bound holds:
\[
\|v\|_{L^\infty(0,T; H)} \lesssim \|\bar{u}\|_{L^2(0,T; H)}.
\]
Additionally, $v(t')=0$, which will be particularly beneficial in the limiting analysis. \\
\indent We next test \eqref{ibvp_diff_u} with $v$ defined in \eqref{test_function} and integrate over $(0,T)$. Noting that $\bar{u}(0)=\bar{u}_t(0)=0$, we obtain
\begin{equation}
\begin{aligned}
&   \int_0^{t'} \intO \aaa(u) \bar{u}_t \bar{u} \dxs  -c^2 \int_0^{t'} \intO \nabla v_t \cdot \nabla v \dxs  +\delta \int_0^{t'}\intO |\nabla \bar{u} |^2 \dxs \\
=&\, \begin{multlined}[t]
-	\int_0^{t'} \intO \left\{ 2k_1 (\bar{u}\ut^\tau)_t +\taua \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t  \right\} v \dxs. 
	\end{multlined}
\end{aligned}
\end{equation}
From here we have 
\begin{equation} \label{est_ubar}
	\begin{aligned}
		&   \frac12 \|\sqrt{\aaa}\bar{u}(t')\|^2_{L^2} + \frac{c^2}{2} \|\nabla v(0)\|^2_{L^2}+ \delta \int_0^{t'}\|\nabla \bar{u} (s)\|_{L^2}^2 \ds \\
		=&\, \begin{multlined}[t]
k_1 \int_0^{t'}\intO \ut \bar{u}^2\dxs-2k_1	\int_0^{t'} \intO (\bar{u}\ut^\tau)_tv \dxs\\-\taua 	\int_0^{t'} \intO \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t   v \dxs. 
		\end{multlined}
	\end{aligned}
\end{equation}
We next wish to estimate the second and third term on the right-hand side (the first one will be taken care of by Gronwall's inequality).  We have for any $\varepsilon>0$
\begin{equation}
	\begin{aligned}
		-2k_1\int_0^{t' }\intO   (\bar{u}\ut^\tau)_tv \dxs 
		=&\, -2k_1\int_0^{t' }\intO   \ut^\tau \bar{u}^2\dxs   \\
		\lesssim&\,  \|u_t^\tau\|_{L^\infty(L^4)}\|\bar{u}\|_{L^2(L^2)}\|\bar{u}\|_{L^2(L^4)} \\
		\lesssim&\,  \|u_t^\tau\|_{L^\infty(L^4)}^2\|\bar{u}\|_{L^2(L^2)}^2 + \varepsilon \|\nabla \bar{u}\|^2_{L^2(L^2)}.
	\end{aligned}
\end{equation}
We recall that $\|u_t^\tau\|_{L^\infty(L^4)} \leq C$ uniformly in $\tau$.  Since the test function is zero at $t'$,  we have
\begin{equation}
	\begin{aligned}
		- \int_0^{t' }\intO \taua \frakKone*\uttt^\tau v \dxs
	%	=&\, -\int_0^{t' }\intO \taua (\frakKone*\utt^\tau)_t v \dxs + \inttO \taua \frakKone(s)u_2 v \dxs  \\
		=&\, \, \begin{multlined}[t] \taua  \left\{ %\intO(\frakKone*\utt^\tau)(0) v(0)\dx+
			\int_0^{t' }\intO  \frakKone*\utt^\tau  v_t \dxs \right.  \left.+ \int_0^{t' }\intO  \frakKone(s)u_2 v \dxs\right\}
		\end{multlined}\\
			=&\, \, \begin{multlined}[t] \taua  \left\{ %\intO(\frakKone*\utt^\tau)(0) v(0)\dx+
	-	\int_0^{t' }\intO  \frakKone*\utt^\tau  \bar{u}\dxs \right.  \left.+ \int_0^{t' }\intO  \frakKone(s)u_2 v \dxs\right\},
	\end{multlined}
	\end{aligned}
\end{equation}
which can be further bounded as follows:
\begin{equation}
\begin{aligned}
	&\taua  \left\{ %\intO(\frakKone*\utt^\tau)(0) v(0)\dx+
	-	\int_0^{t' }\intO  \frakKone*\utt^\tau  \bar{u}\dxs \right.  \left.+ \int_0^{t' }\intO  \frakKone(s)u_2 v \dxs\right\}\\
	 \lesssim&\, \tau^{2a}\|\frakKone*\utt^\tau\|^2_{L^2(L^2)}+\|\bar{u}\|^2_{L^2(L^2)}+ \tau^{2a}\|\frakKone\|_{L^1(0,T)} \|u_2\|_{L^2(\Omega)} \|v\|_{L^\infty(L^2)}\\
	  \lesssim&\, \tau^{2a} \|\frakKone*\utt^\tau\|^2_{L^2(L^2)}+\|\bar{u}\|^2_{L^2(L^2)}+ \tau^{2a}\|\frakKone\|^2_{L^1(0,T)} \|u_2\|_{L^2(\Omega)}^2 .
\end{aligned}
\end{equation}
Additionally,
\begin{equation}
\begin{aligned}
\taua c^2	\int_0^{t'} \intO \frakKone * \Delta u^\tau_t   v \dxs \lesssim&\, \taua \|\frakKone\|_{L^1(0,T)}\|\nabla \ut^\tau\|_{L^2(L^2)}\|\nabla v\|_{L^2(L^2)} \\
\lesssim& \tau^{2a} \|\frakKone\|_{L^1(0,T)}^2\|\nabla \ut^\tau\|_{L^2(L^2)}^2+\varepsilon \|\nabla v\|_{L^2(L^2)}^2.
\end{aligned}
\end{equation}
We can use these bounds to further estimate the right-hand side terms in \eqref{est_ubar} and then employ Gronwall's inequality. In this manner, we arrive at the following result.
\begin{theorem}[Limiting strong behavior of equations with Westevelt-type nonlinearities]\label{Thm:StrongLim_West}
Let the assumptions of Proposition~\ref{Prop:WeakLim_West} hold. Let $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ be the family of solutions to \eqref{weak_GFE_tau}
and let $u$ be the solution of the corresponding limiting problem for the Westervelt equation with $\tau=0$. Then 
\begin{equation}
\|u-u^\tau\|_{L^\infty(L^2)}  +  \left\{\int_0^{T}\|\nabla (u-u^\tau)(s)\|_{L^2}^2\ds\right\}^{1/2} \leq  C \taua,
\end{equation}
where the constant $C>0$ does not depend on $\tau$.
\end{theorem}
This theorem shows that the nonlocal equation 
\begin{equation}
\taua \frakKone *(\utt-c^2\Delta u)_t+ ((1+2k_1 u) \ut)_t-c^2\bbb\Delta u - \delta \Delta \ut  = f
\end{equation}
 can be seen as an approximation of the strongly damped Westervelt equation for small enough relaxation time, under the stated assumptions on the kernel. Indeed, by Theorem~\ref{Thm:StrongLim_West}, solutions of the nonlocal problem converge to the solutions of the limiting problem with the order $a$ in the norm of the space $L^\infty(0,T; L^2(\Omega)) \cap L^2(0,T; \Honezero)$.
 \begin{remark}[On the convergence in the energy norm]
 	The main obstacle to obtaining convergence in the energy norm is the lack of a uniform bound on $\|\utt\|_{L^\infty(L^2)}$ with respect to the relaxation time. To obtain it, an idea might be to differentiate equation \eqref{GFE_type_eq} and perform an analogous testing procedure to before by testing it with $y_t=(\utt-c^2 \Delta u)_t$. However, the issue is that we would need to first ensure the boundedness of $\uttt(0)$ to write the leading term of the time-differentiated equation in the form of $\frakKone*(u_{ttt}-c^2 \Delta \ut)_t$ suitable for such testing.
 \end{remark}
\section{Analysis with Blackstock--Kuznetsov-type nonlinearities}  The ideas put forward in the previous section can be extended to work for more general nonlinearites. Again, we first outline the key ideas before justifying them rigorously. In this section, the linearized equation has the form
\begin{equation} \label{linear_eq_higher}
	\taua \frakKone *(\utt-c^2\Delta u)_t+ \aaa(x,t) \utt-c^2\bbb(x,t)\Delta u - \delta \Delta \ut = \calF(x,t)
\end{equation}
where we think of the coefficient $\aaa$ as a placeholder for $1+2k_1 \ut$, the coefficient $\bbb$ for $1-2k_2 \ut$, and the source term $\calF$ for
 \[
-2 \ell \nabla u\cdot \nabla \ut +f. 
\]
To treat such Blackstock- and Kuznetsov-type nonlinearities, we need more smoothness of the solution compared to before. Therefore, here we test (in a smooth semi-discrete setting) the linearized equation
 with \[-\Delta y= -\Delta (\utt-c^2\Delta u).\]
  Let $\calF \in L^2(0,T; H^1(\Omega))$. 
 By using again the coercivity of the kernel $\frakKone$ assumed in \eqref{eqn:Alikhanov_1}, this approach leads to
\begin{equation} \label{higher_testing_GFE}
	\begin{aligned}
		&\inttO	\nabla( \aaa \utt-c^2\bbb\Delta u - \delta \Delta \ut) \cdot \nabla (\utt-c^2\Delta u)\dxs\\
		\leq& \, \intt \| \calF(s) \|_{H^1} \|\utt(s)-c^2\Delta u(s)\|_{H^1}\ds+ \taua C_{\frakKone} \|\nabla \utt(0)-c^2 \nabla \Delta u(0)\|^2_{L^2}.
	\end{aligned}
\end{equation}
Above we have relied on the trace theorem to treat the $\calF$ term:
\begin{equation}
\begin{aligned}
\left|\intO \calF (-\Delta y) \dxs \right| =&\, \left| \intO \nabla \calF \cdot \nabla y \dxs - \int_{\partial \Omega} \frac{\partial y}{\partial n} \calF \dx \textup{d}\Gamma \right|\\
\leq&\, \|\nabla \calF\|_{L^2} \|\nabla y\|_{L^2}+\left\| \frac{\partial y}{\partial n}\right\|_{H^{-1/2}(\partial \Omega)}\|\calF\|_{H^{1/2}(\partial \Omega)} 
\lesssim\, \|\calF\|_{H^1}\|y\|_{H^1}.
\end{aligned}
\end{equation}
From \eqref{higher_testing_GFE} we then have
\begin{equation}
	\begin{aligned}
&\begin{multlined}[t]\int_0^t\|\sqrt{\aaa(s)} \nabla \utt(s)\|^2_{L^2} \ds+\frac{\delta c^2}{2}\|\nabla \Delta u(s)\|^2_{L^2}\Big \vert_0^t+\frac{\delta}{2}\|\Delta u_t(s)\|^2_{L^2} \Big \vert_0^t \end{multlined} \\
\leq&\, \begin{multlined}[t]-c^4 \int_0^t \bbb |\nabla \Delta u|^2\dxs  -\inttO \utt \nabla \aaa \cdot \nabla \utt \dxs+c^2 \inttO \nabla (\aaa \utt) \cdot \nabla \Delta u \dxs\\ +c^2 \inttO \nabla (\bbb \Delta u) \cdot \nabla \utt \dxs 
-	c^4 \inttO \Delta u \nabla \bbb  \cdot \nabla \Delta u \dxs\\+\intt \| \calF \|_{H^1} \|\utt-c^2\Delta u\|_{H^1}\ds 
+ \taua C_{\frakKone} \|\nabla \utt(0)-c^2 \nabla \Delta u(0)\|^2_{L^2}. \end{multlined}
	\end{aligned}
\end{equation}
Besides sufficient smoothness of $\aaa$ and $\bbb$, and non-degeneracy of $\aaa$, we also need smallness of the coefficients in the following sense:
\begin{equation} \label{smallness_m}
	\begin{aligned}
		\|\nabla \aaa\|_{L^\infty(L^4)}+ \|\nabla \bbb\|_{L^1(L^4)} \leq m. 
	\end{aligned}
\end{equation}
Then we have
\begin{equation} \label{higher_order_est}
	\begin{aligned}
	&\begin{multlined}[t] \|\nabla \Delta u(t)\|^2_{L^2}+\|\Delta u_t(t)\|^2_{L^2}  + \int_0^t\| \nabla \utt\|^2_{L^2}\ds\end{multlined} \\
	\lesssim_T&\, \begin{multlined}[t] \|\nabla \Delta u_0\|^2_{L^2}+\|\Delta u_1\|^2_{L^2} +\taua \|\nabla u_2\|^2_{L^2} + \| \calF\|^2_{L^2(H^1)}. \end{multlined}
	\end{aligned}
\end{equation}
Thus the solution space is
	\begin{equation} \label{def_calU_GFE_higher}
	u \in \calUGFE_{\text{higher}} = L^\infty(0,T; \Honethree) \cap W^{1, \infty}(0,T; \Honetwo) \cap H^2(0,T; \Honezero).
\end{equation} 
We formalize the above arguments with the following well-posedness result in $\calUGFE_{\text{higher}}$. 
\begin{proposition}\label{Prop:Wellp_GFE_lin_higher}
	Let $T>0$, $\delta>0$, and $\tau \in (0, \bar{\tau}]$. Let  $\frakKone \in L^1(0,T)$ and let assumption \eqref{eqn:Alikhanov_1} on the kernel $\frakKone$ hold. Furthermore, assume that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone*\tfrakKone=1$. Let the coefficients $\aaa$ and $\bbb$ satisfy 
\begin{equation}
\begin{aligned}
	&\aaa \in  L^\infty(0,T; L^\infty(\Omega) \cap W^{1,4}(\Omega)),\\
	&\bbb \in  L^\infty(0,T; L^\infty(\Omega)) \cap L^1(0,T; W^{1,4}(\Omega)).
\end{aligned}
\end{equation}
Assume that $\aaa$ does not degenerate so that \eqref{nondeg_aaa} holds. Let $\calF \in L^2(0,T; H^1(\Omega))$ and
\begin{equation}
\begin{aligned}
			(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2) \in \Honethree \times \Honetwo \times \Honezero.
\end{aligned}
\end{equation}
	Then there exists $m>0$, independent of $\tau$, such that if the smallness condition \eqref{smallness_m} holds,
	then there is a unique solution $	u \in \calUGFE_{\text{higher}}$ of the following problem:
	\begin{equation} \label{IBVP_Westtype_lin_higher}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t+\aaa(x,t) u_{tt}
			-c^2 \bbb(x,t) \Delta u -\delta \Delta \ut= \calF(x,t),\end{multlined}\\
		&u\vert_{\partial \Omega}=0, \\
		&	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2).
	\end{aligned} \right. 
\end{equation}  The solutions satisfies 
	\begin{equation}\label{final_est_GFE_lin}
		\begin{aligned}
			\|u\|_{\calUGFE_{\textup{higher}}}^2 \lesssim_T \|u_0\|^2_{H^3}+\|u_1\|^2_{H^2} + \tau^a  \|u_2\|^2_{H^1}+ \|\calF\|_{L^2(H^1)}^2,
		\end{aligned}
	\end{equation}
	where the hidden constant has the form
	\begin{equation}
		C_{\textup{lin}, \textup{higher}} = C \exp \{(1+\|\aaa\|^2_{W^{1,\infty}(L^4)}+\|b\|_{L^\infty(L^\infty)}+\|\bbb\|^2_{L^1(W^{1,4})})T\}.
	\end{equation}
	and does not depend on $\tau.$ 
\end{proposition}
\begin{proof}
The core of the arguments is contained in the above energy analysis leading up to \eqref{higher_order_est} which can be made rigorous through the Galerkin procedure as before. We omit these details here. \\
\indent By boostrapping, we also obtain a uniform bound on
\begin{equation}
	\begin{aligned}
	\taua	\|\frakKone * (\utt-c^2 \Delta u)_t\|_{L^2(L^2)} \leq C.
	\end{aligned}	
\end{equation}
\indent We note that the uniqueness of the constructed solution may be shown by testing the homogeneous problem by $y= \utt-\Delta u$, which is a valid test function in this setting.
\end{proof}
To connect this result to the nonlinear problem, we employ again the Banach fixed-point theorem, this time  to the mapping
 \begin{equation}
	\begin{aligned}
		T: \calB_{\text{higher}} \ni u^* \mapsto u, 
	\end{aligned}
\end{equation}
where $u$ solves \eqref{IBVP_Westtype_lin_higher} with
\begin{equation}
	\begin{aligned}
		\aaa(u^*) =&\,1+2k_1 u_t^*, \quad \bbb = 1-2k_2 u_t^*, \\
		\calF(x,t)= &\,  - \calN(\nabla u^*, \nabla u^*_t)+ f(x,t)= - 2\ell \nabla u^*\cdot \nabla u_t^*+ f(x,t),
	\end{aligned}
\end{equation}
and $u^*$ is taken from the ball
\begin{equation}
	\begin{aligned}
		\calB_{\text{higher}} =\left \{ u \in \calUGFE_{\text{higher}}:\right.&\, \, \|u\|_{\calUGFE_{\text{higher}}} \leq R,\ %\|2k_1 \nabla u+2k_2 \nabla \ut\|_{L^\infty(L^4)} \leq m, \\&\,  \|k_1 u+k_2u_t\|_{L^\infty(L^\infty)} \leq \frac{1}{2 },\\
		\left	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2) \}, \right.
	\end{aligned}
\end{equation}
where the radius $R>0$ will be chosen as small enough in the proof, independently of $\tau$.  
\begin{theorem}[Uniform well-posedness of equations with Blackstock--Kuznetsov-type nonlinearities]\label{Thm:WellP_GFE_BlckstockKuznetov} 
	Let $T>0$ and $\tau \in (0, \bar{\tau}]$. Let $c$, $\delta>0$ and $k_1$, $k_2$, $\ell \in \R$. Let assumption \eqref{eqn:Alikhanov_1} on the kernel $\frakKone$ hold. Furthermore, assume that there exists $\tfrakKone \in L^2(0,T)$, such that $\frakKone * \tfrakKone =1$. Let
	\begin{equation}
		(u_0, u_1, u_2) \in  \Honethree \times \Honetwo \times  \Honezero
	\end{equation}
	and $f \in L^2(0,T; H^1(\Omega))$. There exists $r>0$, independent of $\tau$, such that if
	\begin{equation}
		\|u_0\|^2_{H^3}+\|u_1\|^2_{H^2} + \bar{\tau}^a C(\frakKone) \|u_2\|^2_{H^1}+ \|f\|^2_{L^2(H^1)} \leq r^2,
	\end{equation}
	then there is a unique solution $u \in \calB_{\text{higher}}$ of the nonlinear problem
	\begin{equation} \label{IBVP_BlackstockKuznetsov_type}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt-c^2 \Delta u)_t+(1+2k_1 u_t) u_{tt}
			-c^2 (1-2k_2 u_t)\Delta u -\delta \Delta \ut\\+ 2 \ell \nabla u \cdot \nabla u_t=f(x,t) \quad \text{in }\ \Omega\times (0,T), \end{multlined}\\
		&u\vert_{\partial \Omega}=0, \\
		&	(u, u_t, u_{tt})\vert_{t=0} =(u_0, u_1, u_2).
	\end{aligned} \right. 
\end{equation}
The solution depends continuously on the data with respect to the $\|\cdot\|_{\calUGFE_{\text{higher}}}$ norm.
\end{theorem}
\begin{proof}
The proof can be conducted similarly to the proof of Theorem~\ref{Thm:WellP_GFE}, so we only point out the main differences. The smallness of the coefficients can be guaranteed by noting that
\begin{equation}
\begin{aligned}
	\|\nabla \aaa\|_{L^\infty(L^4)}+ \|\nabla \bbb\|_{L^1(L^4)} \lesssim_T 	\|\nabla u_t^*\|_{L^\infty(L^4)} 
	 \lesssim_T	\|u_t^*\|_{L^\infty(H^2)}  \lesssim R
\end{aligned}
\end{equation}
and then reducing $R$ so that the right-hand side is smaller than $m$. The self-mapping property for $T$ can be obtained similarly to before by noting that
	\begin{equation}
		\begin{aligned}
		\|	\calF\|_{L^2(H^1)} \lesssim&\,  \|\nabla u^*\cdot \nabla u_t^*\|_{L^2(H^1)}+ \|f\|_{L^2(H^1)} \\
		\lesssim&\, \begin{multlined}[t] \|\nabla u^*\|_{L^\infty(L^4)}\| \nabla u_t^*\|_{L^2(L^4)}+\|\nabla u^*\|_{L^\infty(L^\infty)} \| \nabla^2 u_t^*\|_{L^2(L^2)}\\+\|\nabla^2 u^*\|_{L^\infty(L^4)} \| \nabla u_t^*\|_{L^2(L^4)}+ \|f\|_{L^2(H^1)} \end{multlined}\\
			\lesssim&\, \begin{multlined}[t] \| u^*\|_{L^\infty(H^2)}\|  u_t^*\|_{L^2(H^2)}+\| u^*\|_{L^\infty(H^3)} \|  u_t^*\|_{L^2(H^2)}\\+\|u^*\|_{L^\infty(H^3)} \|  u_t^*\|_{L^2(H^2)}+ \|f\|_{L^2(H^1)}
			\end{multlined}\\
		\lesssim&\, R^2+ \|f\|_{L^2(H^1)}.
		\end{aligned}
	\end{equation}
Finally, let us discuss the strict contractivity. Let $T u^{*} =u$ and $T v^*=v$. We denote their differences by $\phi=u-v$ and $\phi^*= u^*-v^*$. Then $\phi$ is a solution of the following equation:
\begin{equation}\label{diff_eq_contractivity_BK}
	\begin{aligned}
		{\tau^a}  \frakKone *( \phi_{tt}-c^2\Delta \phi)_t+\aaa(u_t^*) \phi_{t}
			-c^2   \bbb(u^*_t) \Delta \phi
			-   \delta   \Delta \phi_{t}= \calF
	\end{aligned}
\end{equation}
with the right-hand side
\begin{equation}
	\begin{aligned}
	\calF
		=&\, -(\aaa(u_t^*)-\aaa(v_t^*)) v_{tt} +c^2(\bbb(u_t^*)-\bbb(v_t^*)) \Delta v-(\calN(\nabla u^*, \nabla u^*_t) -\calN(\nabla v^*, \nabla v^*_t))\\
		=&\, -2k_1 \phi_t^* v_{tt} +2k_2c^2 \phi^*_t\Delta v +2\ell \nabla \phi^* \cdot(\nabla u_t^*+\nabla v_t^*)+2\ell \nabla \phi^*_t \cdot (\nabla u^*+\nabla v^*)
	\end{aligned}
\end{equation}
and homogeneous boundary and initial conditions. It is straightforward to check that 
\begin{equation}
	\begin{aligned}
		\| \calF\|_{L^2(H^1)} \lesssim  R \|\phi^*\|_{\calUGFE_{\text{higher}}}.
	\end{aligned}
\end{equation}
Thus employing energy estimate \eqref{final_est_GFE_lin} for the solution of \eqref{diff_eq_contractivity_BK} gives
\begin{equation}
	\begin{aligned}
	 \|\phi\|_{\calUGFE_{\text{higher}}} \lesssim   R \|\phi^*\|_{\calUGFE_{\text{higher}}},
	\end{aligned}
\end{equation}
and we can guarantee strict contractivity of the mapping $T>0$ by reducing the radius $R$. An application of Banach's fixed-point theorem yields the desired result.
\end{proof}
\subsection{Limiting weak behavior of equations with Blackstok--Kuznetsov-type nonlinearities} Under the assumptions of Theorem~\ref{Thm:WellP_GFE_BlckstockKuznetov}, we next discuss the vanishing thermal relaxation limit of the family $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ of solutions to the following problem:
\begin{equation} \label{IBVP_GFE_tau_BlackstockKuznetsov}
	\left \{	\begin{aligned}
		&\begin{multlined}[t]	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t+\aaa(u^\tau_t) \utt^\tau
			-c^2 \bbb(u^\tau_t) \Delta u^\tau 
			-\delta   \Delta \ut^\tau+\calN(\nabla u^\tau, \nabla u^\tau_t)=f ,\end{multlined}\\
		&u^\tau\vert_{\partial \Omega}=0, \\
		&	(u^\tau, \ut^\tau, \utt^\tau)\vert_{t=0} =(u_0, u_1, u_2).
	\end{aligned} \right. 
\end{equation}
\indent We can adapt the arguments from Section~\ref{Subsec:Weaklim_tau_GFE}  to prove the weak convergence of this family to the solution of the Blackstock--Kuznetsov equation:
\begin{equation}\label{BK_eq}
	\aaa(u^\tau_t) \utt
	-c^2 \bbb(u_t) \Delta u
	-\delta   \Delta \ut+\calN(\nabla u, \nabla u_t)=f
\end{equation}
as the relaxation time tends to zero. By the previous theorem and the obtained uniform bounds, we conclude that there is a susequence, again not relabeled, such that
\begin{equation} \label{weak_limits_tau_GFE_BK}
	\begin{alignedat}{4} 
		u^\tau&\relbar\joinrel\rightharpoonup u && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honethree),  \\
		\ut^\tau &\relbar\joinrel\rightharpoonup u_t && \quad \text{ weakly-$\star$}  &&\text{ in } &&L^\infty(0,T; \Honetwo),\\
		\utt^\tau &\relbar\joinrel\rightharpoonup u_{tt} && \quad \text{ weakly}  &&\text{ in } &&L^2(0,T; \Honezero).
	\end{alignedat} 
\end{equation}
It remains to prove that $u$ is a solution of the limiting problem. 
\begin{proposition}[Limiting weak behavior of equations with Blackstock--Kuznetsov nonlinearities] \label{Prop:WeakLim_BK} 
	Let the assumptions of Theorem~\ref{Thm:WellP_GFE_BlckstockKuznetov} hold.  Then the family $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ of solutions to \eqref{weak_GFE_tau} converges weakly in the sense of \eqref{weak_limits_tau_GFE_BK} to the solution of the corresponding limiting problem for the Blackstock--Kuznetsov equation \eqref{BK_eq}. 
\end{proposition}
\begin{proof}
 Let $v \in C^\infty([0,T]; C_0^\infty(\Omega))$ with $v(T)=0$. We have with $\bar{u}=u-u^\tau$:
	\begin{equation}\label{weak_limit_baru}
		\begin{aligned}
			&\begin{multlined}[t] \intTO \aaa(\ut) \utt v \dxs+ \intTO  (c^2 \bbb(\ut) \Delta u +\delta \Delta \ut)v \dxs\\
				+\inttO \calN(\nabla u, \nabla \ut) v \dxs-\intTO f v \dxs \end{multlined}\\
			=&	\begin{multlined}[t]  \intTO ( \aaa(u)\bar{u}_{tt}+ 2k_1\bar{u}\utt^\tau)  v \dxs+ c^2 \intTO  (\bbb(u)\Delta \bar{u}-2k_2 \bar{u}_t \Delta u^\tau) v \dxs \\+ \delta \intTO  \Delta \bar{u}_{t} v \dxs+ 2\ell \inttO ( \nabla \bar{u}_t \cdot \nabla u+\nabla u^\tau_t\cdot \nabla \bar{u}) v \dxs\\
				- \intTO  \taua \frakKone * (\utt^\tau -c^2 \Delta u^\tau)_t v \dxs.  \end{multlined}
		\end{aligned}
	\end{equation}
We should prove that the right-hand side tends to zero as $\tau \searrow 0$. The main difference compared to the similar analysis before in Proposition~\ref{Prop:WeakLim_West}  comes from treating the nonlinear terms. These can be tackled by exploiting the weak limits in \eqref{weak_limits_tau_GFE_BK} together with the fact that now by the Aubin--Lions--Simon lemma, we have
\begin{equation} \label{weak_limits_tau_GFE_2}
	\begin{alignedat}{4} 
		u^\tau&\longrightarrow u && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Honetwo),  \\
		\ut^\tau &\longrightarrow u_t && \quad \text{ strongly}  &&\text{ in } &&C([0,T]; \Honezero)).
	\end{alignedat} 
\end{equation} 
We omit the details here.  In this manner we obtain a solution of the limitting Blackstock--Kuznetsov problem. \\[2mm]
\noindent \emph{Uniqueness of the solution to the limiting problem.} The uniqueness of solutions to the limiting problem for \eqref{BK_eq} in the Kuznetsov case (that is, with $k_2=0$) follows by \cite[Theorem 4.1]{mizohata1993global} with the right-hand side assumed to be such that
\[
f \in C([0,T]; L^2(\Omega)) \cap L^2(0,T; H^1(\Omega)),\ f_t \in L^2(0,T; H^{-1}(\Omega)).
\]
 In the Blackstock case (that is with $k_1=0$) and with $f=0$, it follows by \cite[Theorem 1]{fritz2018well}. In the general Blackstock--Kuznetsov case \eqref{BK_eq} with a source term considered here, it can be shown by testing the homogeneous equation with $\ut$, for example. Thus by a subsequence-subsequence argument we conclude that the whole sequence $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ converges to $u$ in the sense of \eqref{weak_limits_tau_GFE_BK}.  
\end{proof}
\subsection{Strong convergence with Blackstock-type nonlinearities} To discuss the strong convergence, we see the difference $\bar{u}=u-u^\tau$ as the solution of
\begin{equation} \label{ibvp_diff_u_BK}
	\begin{aligned}
	\begin{multlined}[t]	\aaa(\ut)\bar{u}_{tt}-c^2 \bbb(\ut) \Delta \bar{u} 
		-\delta   \Delta \bar{u}_t=-2k_1 \bar{u}_t \utt^\tau+2 c^2 k_2 \bar{u}_t \Delta u^\tau
		-2\ell \nabla\bar{u}_t \cdot \nabla u\\-2\ell \nabla u^\tau_t \cdot \nabla \bar{u} +	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t 
	\end{multlined}	
	\end{aligned}
\end{equation}
with homogeneous data. However, obtaining strong convergence of solutions as $\tau \searrow 0$ with the order $a$ does not seem feasible using the procedure from before since, after testing with $v$ as in \eqref{test_function}, we would have to further treat the term
\[
-2k_1\inttO \bar{u}_t \utt^\tau v \dxs
\]
by integration by parts to get to a bound on $\bar{u}$ in the $L^\infty(0,T; L^2(\Omega)) \cap L^2(0,T; \Honezero)$ norm. This would result in the third time derivative $\uttt^\tau$ which we cannot control. For this reason we restrict the discussion in this section to the Blackstock-type nonlinearities; that is, we assume that $k_1=0$ and thus $\aaa \equiv 1$ so that in the limit we obtain the Blackstock wave equation. The difference equation above then simplifies to
\begin{equation} \label{ibvp_diff_u_B}
	\begin{aligned}
		\begin{multlined}[t]	\bar{u}_{tt}-c^2 \bbb(\ut) \Delta \bar{u} 
			-\delta   \Delta \bar{u}_t=2 c^2 k_2 \bar{u}_t \Delta u^\tau
			-2\ell \nabla\bar{u}_t \cdot \nabla u-2\ell \nabla u^\tau_t \cdot \nabla \bar{u} \\+	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t.
		\end{multlined}	
	\end{aligned}
\end{equation}
Testing with $v$ as in \eqref{test_function} and integrating over $\Omega$ and $(0,t')$ then leads to 
\begin{equation}\label{v_testing_Blackstock}
	\begin{aligned}
		&   \|\bar{u}(t')\|^2_{L^2}  + \frac{c^2}{2} \|\nabla v(0)\|^2_{L^2}  +\delta \int_0^{t'}\intO |\nabla \bar{u} |^2 \dxs \\
		=&\, \begin{multlined}[t] -2c^2 k_2 \int_0^{t'} \intO \ut \Delta \bar{u} v \dxs\\+ \int_0^{t'}\intO \left\{2 c^2 k_2 \bar{u}_t \Delta u^\tau
			-2\ell \nabla\bar{u}_t \cdot \nabla u-2\ell \nabla u^\tau_t \cdot \nabla \bar{u} \right\} v \dxs
			\\-	\taua\int_0^{t'} \intO  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t   v \dxs. 
		\end{multlined}
	\end{aligned}
\end{equation}
We can treat the convolution term as before so we discuss the remaining terms. First,
\begin{equation}
	\begin{aligned}
	 &\int_0^{t'} \intO \ut \Delta \bar{u} v \dxs\\
	  =&\,   \int_0^{t'} \intO \ut \nabla \bar{u} \cdot \nabla v \dxs+ \int_0^{t'} \intO  \nabla \ut  \cdot \nabla \bar{u} v \dxs \\
		\lesssim&\, \|\ut\|_{L^2(L^\infty)} \|\nabla \bar{u}\|_{L^2(L^2)}\|\nabla v\|_{L^2(L^2)}+ \|\nabla \ut\|_{L^2(L^4)} \|\nabla \bar{u}\|_{L^2(L^2)}\| v\|_{L^\infty(L^4)}\\
			\lesssim&\, \|\ut\|_{L^2(L^\infty)} \|\nabla \bar{u}\|_{L^2(L^2)}^2+ \|\Delta \ut\|_{L^2(L^2)} \|\nabla \bar{u}\|_{L^2(L^2)}^2.
	\end{aligned}
\end{equation}
Next, 
\begin{equation}
	\begin{aligned}
		&\int_0^{t'} \intO  \bar{u}_t \Delta u^\tau v \dxs\\
		 =&\, -\int_0^{t'} \intO  \bar{u} \Delta u_t^\tau v \dxs+\int_0^{t'} \intO  \bar{u}^2 \Delta u^\tau  \dxs\\
		\lesssim&\, \|\Delta u_t^\tau \|_{L^2(L^2)} \|\bar{u}\|_{L^2(L^4)}\|v\|_{L^\infty(L^4)} + \|\Delta u^\tau\|_{L^\infty(L^4)} \|\bar{u}\|_{L^2(L^2)}\|\bar{u}\|_{L^2(L^4)}.
	\end{aligned}
\end{equation}
Finally, we have
\begin{equation}
	\begin{aligned}
&\int_0^{t'} \intO\left\{	-2\ell \nabla\bar{u}_t \cdot \nabla u-2\ell \nabla u^\tau_t \cdot \nabla \bar{u} \right\} v \dxs \\
=&\, 2\ell \int_0^{t'} \intO \nabla\bar{u} \cdot \nabla u_t v \dxs-2\ell \int_0^{t'} \intO \nabla\bar{u} \cdot \nabla u \bar{u} \dxs-2\ell  \int_0^{t'} \intO\nabla u^\tau_t \cdot \nabla \bar{u}v \dxs \\
\lesssim&\, \begin{multlined}[t] \|\nabla \bar{u}\|_{L^2(L^2)}\|v\|_{L^\infty(L^4)}\|\nabla u_t\|_{L^2(L^4)}+\|\nabla \bar{u}\|_{L^2(L^2)}\|\bar{u}\|_{L^2(L^4)}\|\nabla u\|_{L^\infty(L^2)}
	\\+\|\nabla u_t^\tau\|_{L^2(L^4)}\|\nabla \bar{u}\|_{L^2(L^2)}\|v\|_{L^\infty(L^4)}.
	\end{multlined}
	\end{aligned}
\end{equation}
Thus by employing these bounds in \eqref{v_testing_Blackstock} and relying on the established uniform bounds on $u^\tau$ and Gronwall's inequality, we arrive at the following result.  
\begin{theorem}[Limiting strong behavior of equations with Blackstock-type nonlinearities]
	Let the assumptions of Theorem~\ref{Thm:WellP_GFE_BlckstockKuznetov} hold. Let $\{u^\tau\}_{\tau \in (0, \bar{\tau}]}$ be the family of solutions to \eqref{weak_GFE_tau}
	and let $u$ be the solution of the corresponding limiting initial boundary-value problem for the Blackstock equation:
	\begin{equation}\label{B_eq}
	\utt
		-c^2(1-2k_2 \ut) \Delta u
		-\delta   \Delta \ut+2 \ell \nabla u \cdot \nabla \ut=f. 
	\end{equation}
 Then the following estimate holds:
	\begin{equation}
		\|u-u^\tau\|_{L^\infty(L^2)}  +  \left\{\int_0^{T}\|\nabla (u-u^\tau)(s)\|_{L^2}^2\ds\right\}^{1/2} \leq  C \taua,
	\end{equation}
	where the constant $C>0$ does not depend on $\tau$.
\end{theorem}
Thus, provided the kernel and data satisfy the assumptions of Theorem~\ref{Thm:WellP_GFE_BlckstockKuznetov}, we may see equation
\begin{equation}
	{\tau^a}  \frakKone * (\utt^\tau-c^2\Delta u^\tau)_t+ \utt^\tau
	-c^2 (1-2k_2u^\tau_t) \Delta u^\tau 
	-\delta   \Delta \ut^\tau+2\ell \nabla u^\tau \cdot \nabla u^\tau_t=f 
\end{equation}
as an approximation of \eqref{B_eq} for small enough relaxation time. 
\begin{remark}[Further comments on the linear equation with constant coefficients]
If we are in the linear setting with constant coefficients $\aaa=\bbb=1$:
\begin{equation}
\taua \frakKone *(\utt-c^2\Delta u)_t+ \utt-c^2\Delta u - \delta \Delta \ut = \calF,
\end{equation}
the situation simplifies significantly. The previous energy arguments in the well-posedness analysis can also be made uniform with respect to $\delta \in (0, \bar{\delta}]$. Indeed, testing with $y=\utt-c^2\Delta u$ as before leads to the bound
\begin{equation}
\begin{aligned}
\|\utt-c^2\Delta u\|^2_{L^2(L^2)} \lesssim \|\calF\|^2_{L^2(L^2)}+\taua\|u_2\|^2_{L^2}+\|\nabla u_1\|^2_{L^2} +\|\Delta u_0\|^2_{L^2},
\end{aligned}
\end{equation}
where the hidden constant is independent of both $\tau$ and $\delta$. From
\[
\utt-c^2\Delta u =y,
\]
and a uniform bound on $\|y\|_{L^2(L^2)}$, we further have by \cite[Ch.\ 5, Lemma 7]{dautray1992evolution}
\[
\|\utt\|_{L^2(H^{-1})}+ \|\ut\|_{L^\infty(L^2)}+ \|\nabla u\|_{L^\infty(L^2)} \leq C,
\]
where again $C>0$ does not depend neither on $\tau$ nor on $\delta$. This bound can then be further used to study the limiting behavior with respect to both parameters.
\end{remark}

\subsection{On the Jordan--Moore--Gibson--Thompson equation}
The uniform and limiting analysis presented above can be modified in a straightforward manner to work for $\frakKone=\delta_0$, that is, for the Jordan--Moore--Gibson--Thompson equation with both types of nonlinearities:
\[
\tau (\utt-c^2 \Delta u)_t + (\aaa \ut)_t-c^2\bbb \Delta u -\delta \Delta \ut +\calN= f,
\]
as the same testing procedure can be applied using $y=\utt-c^2\Delta u$ or $-\Delta y$. \\
\indent For $\aaa=1+2k_1 u$ and $\bbb=1$, $\calN=0$, this complements the available results~\cite{kaltenbacher2019jordan, bongarti2020vanishing} on the limiting analysis for this third-order equation with Westervelt-type nonlinearities by providing strong convergence with order $1$ in $L^\infty(0,T; L^2(\Omega)) \cap L^2(0,T; \Honezero)$ for small data in $\Honetwo \times \Honezero \times L^2(\Omega)$ and $f \in L^2(0,T; L^2(\Omega))$. Strong convergence for Blackstock or Kuznetsov-type nonlinearities has not been considered before, to the best of our knowledge. \gentodo{maybe state as a theorem?}

